Posterior Convergence of Nonparametric Binary and Poisson Regression Under Possible Misspecifications

In this article, we investigate posterior convergence of nonparametric binary and Poisson regression under possible model misspecification, assuming general stochastic process prior with appropriate properties. Our model setup and objective for binary regression is similar to that of Ghosal and Roy (2006) where the authors have used the approach of entropy bound and exponentially consistent tests with the sieve method to achieve consistency with respect to their Gaussian process prior. In contrast, for both binary and Poisson regression, using general stochastic process prior, our approach involves verification of asymptotic equipartition property along with the method of sieve, which is a manoeuvre of the general results of Shalizi (2009), useful even for misspecified models. Moreover, we will establish not only posterior consistency but also the rates at which the posterior probabilities converge, which turns out to be the Kullback-Leibler divergence rate. We also investgate the traditional posterior convergence rates. Interestingly, from subjective Bayesian viewpoint we will show that the posterior predictive distribution can accurately approximate the best possible predictive distribution in the sense that the Hellinger distance, as well as the total variation distance between the two distributions can tend to zero, in spite of misspecifications.

==> supp_gp.tex <==

\renewcommand\thefigure{S-\arabic{figure}}
\renewcommand\thetable{S-\arabic{table}}
\renewcommand\thesection{S-\arabic{section}}
\renewcommand\thetheorem{S-\arabic{theorem}}

\setcounter{section}{0}
\setcounter{theorem}{0}


\begin{center}
{\LARGE\bf Supplementary Material}
\end{center}

\section{Preliminaries for ensuring posterior consistency under general set-up}
\label{sec:shalizi}


Following \ctn{Shalizi09} we consider a probability space $(\Omega,\mathcal F, P)$, 
and a sequence of random variables $y_1,y_2,\ldots$,   
taking values in some measurable space $(\Xi,\mathcal Y)$, whose
infinite-dimensional distribution is $P$. The natural filtration of this process is
$\sigma(\by_n)$. %where $\bY_n=(Y_1,Y_2,\ldots,Y_n)^T$.

We denote the distributions of processes adapted to $\sigma(\by_n)$ 
by $F_{\theta}$, where $\theta$ is associated with a measurable
space $(\Theta,\mathcal T)$, and is generally infinite-dimensional. 
For the sake of convenience, we assume, as in \ctn{Shalizi09}, that $P$
and all the $F_{\theta}$ are dominated by a common reference measure, with respective
densities $f_0$ and $f_{\theta}$. The usual assumptions that $P\in\Theta$ or even $P$ lies in the support 
of the prior on $\Theta$, are not required for Shalizi's result, rendering it very general indeed.



\subsection{Assumptions and theorems of Shalizi}
\label{subsec:assumptions_shalizi}

\begin{itemize}
\item[(S1)] Consider the following likelihood ratio:
\begin{equation}
R_n(\theta)=\frac{f_{\theta}(\bY_n)}{f_{\theta_0}(\bY_n)}.
\label{eq:R_n}
\end{equation}
Assume that $R_n(\theta)$ is $\sigma(\bY_n)\times \mathcal T$-measurable for all $n>0$.
\end{itemize}

\begin{itemize}
\item[(S2)] For every $\theta\in\Theta$, the KL-divergence rate
\begin{equation}
h(\theta)=\underset{n\rightarrow\infty}{\lim}~\frac{1}{n}E\left(\log\frac{f_{\theta_0}(\bY_n)}{f_{\theta}(\bY_n)}\right).
\label{eq:S3}
\end{equation}
exists (possibly being infinite) and is $\mathcal T$-measurable.
\end{itemize}

\begin{itemize}
\item[(S3)] For each $\theta\in\Theta$, the generalized or relative asymptotic equipartition property holds, and so,
almost surely,
\begin{equation*}
\underset{n\rightarrow\infty}{\lim}~\frac{1}{n}\log R_n(\theta)=-h(\theta).
\end{equation*}
\end{itemize}




\begin{itemize}
\item[(S4)] 
Let $I=\left\{\theta:h(\theta)=\infty\right\}$. 
The prior $\pi$ satisfies $\pi(I)<1$.
\end{itemize}

Following the notation of \ctn{Shalizi09}, for $A\subseteq\Theta$, let
\begin{align}
h\left(A\right)&=\underset{\theta\in A}{\mbox{ess~inf}}~h(\theta);\label{eq:h2}\\
J(\theta)&=h(\theta)-h(\Theta);\label{eq:J}\\
J(A)&=\underset{\theta\in A}{\mbox{ess~inf}}~J(\theta).\label{eq:J2}
\end{align}
\begin{itemize}
\item[(S5)] There exists a sequence of sets $\mathcal G_n\rightarrow\Theta$ as $n\rightarrow\infty$ 
such that: %along with $\pi(\mathcal G_T)>0$
\begin{enumerate}
\item[(1)]
\begin{equation}
\pi\left(\mathcal G_n\right)\geq 1-\alpha\exp\left(-\beta n\right),~\mbox{for some}~\alpha>0,~\beta>2h(\Theta);
\label{eq:S5_1}
\end{equation}
\item[(2)]The convergence in (S3) is uniform in $\theta$ over $\mathcal G_n\setminus I$.
\item[(3)] $h\left(\mathcal G_n\right)\rightarrow h\left(\Theta\right)$, as $n\rightarrow\infty$.
\end{enumerate}
\end{itemize}
For each measurable $A\subseteq\Theta$, for every $\delta>0$, there exists a random natural number $\tau(A,\delta)$
such that
\begin{equation}
n^{-1}\log\int_{A}R_n(\theta)\pi(\theta)d\theta
\leq \delta+\underset{n\rightarrow\infty}{\lim\sup}~n^{-1}
\log\int_{A}R_n(\theta)\pi(\theta)d\theta,
\label{eq:limsup_2}
\end{equation}
for all $n>\tau(A,\delta)$, provided 
$\underset{n\rightarrow\infty}{\lim\sup}~n^{-1}\log\pi\left(\mathbb I_A R_n\right)<\infty$.
%$\mathbb I_A$ denotes the indicator function of the set $A$.
Regarding this, the following assumption has been made by Shalizi:
\begin{itemize}
\item[(S6)] The sets $\mathcal G_n$ of (S5) can be chosen such that for every $\delta>0$, the inequality
$n>\tau(\mathcal G_n,\delta)$ holds almost surely for all sufficiently large $n$.
\end{itemize}
\begin{itemize}
\item[(S7)] The sets $\mathcal G_n$ of (S5) and (S6) can be chosen such that for any set $A$ with $\pi(A)>0$, 
\begin{equation}
h\left(\mathcal G_n\cap A\right)\rightarrow h\left(A\right),
\label{eq:S7}
\end{equation}
as $n\rightarrow\infty$.
\end{itemize}
Under the above assumptions, \ctn{Shalizi09} proved the following results.

\begin{theorem}[\ctn{Shalizi09}]
\label{theorem:shalizi1}
Consider assumptions (S1)--(S7) and any set $A\in\mathcal T$ with $\pi(A)>0$ and $h(A)>h(\Theta)$. Then,
\begin{equation*}
\underset{n\rightarrow\infty}{\lim}~\pi(A|\bY_n)=0~\mbox{almost surely},
%\label{eq:supp_post_conv1}
\end{equation*}
where $\pi(\cdot|\bY_n)$ denotes the posterior distribution of $\theta$ given $\bY_n$.
\end{theorem}

The rate of convergence of the log-posterior is given by the following result. 
\begin{theorem}[\ctn{Shalizi09}]
\label{theorem:shalizi2}
Consider assumptions (S1)--(S7) and any set $A\in\mathcal T$ with $\pi(A)>0$. If $\beta>2h(A)$, where
$\beta$ is given in (\ref{eq:S5_1}) under assumption (S5), or if $A\subset\cap_{k=n}^{\infty}\mathcal G_k$ for some $n$, then
\begin{equation*}
\underset{n\rightarrow\infty}{\lim}~\frac{1}{n}\log\pi(A|\bY_n)=-J(A),
%\label{eq:supp_post_conv2}
\end{equation*}
where $\pi(\cdot|\bY_n)$ denotes the posterior distribution of $\theta$ given $\bY_n$.
\end{theorem}
%We shall frequently make use of these theorems for our purpose.

\section{Verification of the assumptions of Shalizi for the Gaussian process model with normal errors}
\label{sec:verification}

\subsection{Verification of (S1)}
\label{subsec:S1}
note that
\begin{align}
f_{\theta}(\bY_n)&=\frac{1}{\left(\sigma\sqrt{2\pi}\right)^n}\exp\left\{-\frac{1}{2\sigma^2}\sum_{i=1}^n(Y_i-\eta(\bx_i))^2\right\};\label{eq:like1}\\
f_{\theta_0}(\bY_n)&=\frac{1}{\left(\sigma_0\sqrt{2\pi}\right)^n}\exp\left\{-\frac{1}{2\sigma^2_0}\sum_{i=1}^n(Y_i-\eta_0(\bx_i))^2\right\}.\label{eq:true_like1}
\end{align}
The equations (\ref{eq:like1}) and (\ref{eq:true_like1}) yield, in our case,
\begin{equation}
\frac{1}{n}\log R_n(\theta)=\log\left(\frac{\sigma_0}{\sigma}\right)+\frac{1}{2\sigma^2_0}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2
-\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta(\bx_i)\right)^2.
\label{eq:R1}
\end{equation}
We show that the right hand side of (\ref{eq:R1}), which we denote as $f(\by_n,\theta)$, is continuous in $(\by_n,\theta)$, which is sufficient to confirm measurability of $R_n(\theta)$.
Let $\|(\by_n,\theta)\|=\|\by_n\|+\|\theta\|$, where $\|\by_n\|$ is the Euclidean norm and $\|\theta\|=\|\eta\|+|\sigma|$, with
$\|\eta\|=\underset{\bx\in\mathcal X}{\sup}~|\eta(\bx)|$. Since $\mathcal X$ is compact and $\eta$ is almost surely continuous, it follows that $\|\eta\|<\infty$ almost surely.

Consider $\by_{n}=(y_{1},y_{2},\ldots,y_{n})^T$ %$\by_{2n}=(y_{21},y_{22},\ldots,y_{2n})^T$, $\theta_1$ and $\theta_2$. 
%such that, given $\varepsilon>0$, $\|(\by_{1n},\theta_1)-(\by_{2n},\theta_2)\|<\frac{\varepsilon}{c}$, for some finite $c>0$.
and $\boeta_{0n}=(\eta_0(\bx_1),\ldots,\eta_0(\bx_n))^T$. 
Then
\begin{equation}
\sum_{i=1}^n(y_{i}-\eta_0(\bx_i))^2=\by^T_n\by_n-2\by^T_n\boeta_{0n}+\boeta^T_{0n}\boeta_{0n}
\label{eq:cont2}
\end{equation}
is clearly continuous in $\by_n$.
%\begin{align}
%&\Bigg|\frac{1}{n}\sum_{i=1}^n(y_{1i}-\eta_0(\bx_i))^2-\frac{1}{n}\sum_{i=1}^n(y_{2i}-\eta_0(\bx_i))^2\Bigg |\notag\\%\label{eq:cont1}\\
%&=\frac{1}{n}\Bigg |\sum_{i=1}^n\left[(y_{1i}-y_{2i})\left\{(y_{1i}-\eta_0(\bx_i))+(y_{2i}-\eta_0(\bx_i))\right\}\right]\Bigg |\notag\\
%&\ \ \leq\|\by_{1n}-\by_{2n}\|\times\left(\frac{\|\by_{1n}-\boeta_{0n}\|}{n}+\frac{\|\by_{2n}-\boeta_{0n}\|}{n}\right).
%\label{eq:cont2}
%\end{align}
%Now note that for $j=1,2$, $\by_{jn}-\boeta_{0n}=\be_{jn}$, where $\be_{jn}=(\e_{j1},\ldots,\e_{jn})^T$ are the $iid$ Gaussian random errors with mean zero and variance $\sigma^2_0$.
%Since the elements of $\be_{jn}$ are almost surely finite, it follows that for $j=1,2$, $\frac{\|\by_{jn}-\boeta_{0n}\|}{n}=
%\sqrt{\sum_{i=1}^n\left(\frac{\e_{ji}}{n}\right)^2}$ is finite. 
%Let $c_1=\sum_{j=1}^2\sqrt{\sum_{i=1}^n\left(\frac{\e_{ji}}{n}\right)^2}$.
%Hence it follows from (\ref{eq:cont2}) that if $\|\by_{1n}-\by_{2n}\|<\frac{\varepsilon}{c_1}$, 
%then (\ref{eq:cont1}) is less than $\varepsilon$, which proves 
%Hence, continuity of the term $\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2$ follows from (\ref{eq:cont2}).
%
Now note that 
\begin{equation}
\frac{1}{n}\sum_{i=1}^n(y_i-\eta(\bx_i))^2=\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))^2+\frac{1}{n}\sum_{i=1}^n(\eta(\bx_i)-\eta_0(\bx_i))^2
-\frac{2}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta(\bx_i)-\eta_0(\bx_i)),
\label{eq:breakup2}
\end{equation}
where we have already proved continuity of the first term on the right hand side of (\ref{eq:breakup2}). %$\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))^2$.
To see continuity of $\frac{1}{n}\sum_{i=1}^n(\eta(\bx_i)-\eta_0(\bx_i))^2$ with respect to $\eta$, first consider any sequence $\left\{\eta_j:j=1,2,\ldots\right\}$ satisfying
$\|\eta_j-\tilde\eta\|\rightarrow 0$, as $j\rightarrow\infty$. Then
\begin{align}
&\Bigg|\frac{1}{n}\sum_{i=1}^n(\eta_j(\bx_i)-\eta_0(\bx_i))^2-\frac{1}{n}\sum_{i=1}^n(\tilde\eta(\bx_i)-\eta_0(\bx_i))^2\Bigg |\label{eq:cont3}\\
&\ \ \leq\frac{1}{n}\sum_{i=1}^n\left|\eta_j(\bx_i)-\tilde\eta(\bx_i)\right|\times\left|(\eta_j(\bx_i)-\eta_0(\bx_i))+(\tilde\eta(\bx_i)-\eta_0(\bx_i))\right|\notag\\
&\ \ \leq\|\eta_j-\tilde\eta\|\times\left[\|\eta_j-\eta_0\|+\|\tilde\eta-\eta_0\|\right]\notag\\
&\ \ \leq\|\eta_j-\tilde\eta\|\times\left[\|\eta_j-\tilde\eta\|+2\|\tilde\eta-\eta_0\|\right]\notag\\
&\ \ \rightarrow 0,~\mbox{as}~j\rightarrow\infty.
\label{eq:cont4}
\end{align}
%Due to continuity of $\eta_0$, $\eta_1$ and $\eta_2$, and compactness of $\mathcal X$, $\|\eta_j-\eta_0\|\leq \|\eta_j\|+\|\eta_0\|<\infty$, for $j=1,2$.
%Letting $c_2=\|\eta_1-\eta_0\|+\|\eta_2-\eta_0\|$, it follows that if $\|\eta_1-\eta_2\|<\frac{\varepsilon}{c_2}$, then (\ref{eq:cont3}) is less than $\varepsilon$,
This proves continuity of the second term of (\ref{eq:breakup2}). 

For the third term of (\ref{eq:breakup2}) we now prove that for any $\tilde \by\in\mathbb R^n$, and for any sequence 
$\left\{\by_j:j=1,2,\ldots\right\}$ (we denote the $i$-th component of $\by_j$ as $y_{ij}$) such that
$\|\by_j-\tilde\by\|\rightarrow 0$, as $j\rightarrow\infty$, and for any function $\tilde\eta$ associated with any sequence $\left\{\eta_j:j=1,2,\ldots\right\}$ satisfying
$\|\eta_j-\tilde\eta\|\rightarrow 0$, as $j\rightarrow\infty$, $\sum_{i=1}^n(y_{ij}-\eta_0(\bx_i))(\eta_j(\bx_i)-\eta_0(\bx_i))\rightarrow
\sum_{i=1}^n(\tilde y_i-\eta_0(\bx_i))(\tilde\eta(\bx_i)-\eta_0(\bx_i))$, as $j\rightarrow\infty$.
Indeed, observe that
\begin{align}
&\Bigg|\sum_{i=1}^n(y_{ij}-\eta_0(\bx_i))(\eta_j(\bx_i)-\eta_0(\bx_i))-\sum_{i=1}^n(\tilde y_i-\eta_0(\bx_i))(\tilde\eta(\bx_i)-\eta_0(\bx_i))\Bigg|\notag\\
&\qquad =\Bigg|\sum_{i=1}^n(y_{ij}-\tilde y_i)(\eta_j(\bx_i)-\tilde\eta(\bx_i))
+\sum_{i=1}^n(\tilde y_i-\eta_0(\bx_i))(\eta_j(\bx_i)-\tilde\eta(\bx_i))\notag\\
&\qquad\qquad +\sum_{i=1}^n(y_{ij}-\tilde y_i)(\tilde\eta(\bx_i)-\eta_0(\bx_i))\Bigg|\notag\\
&\qquad\leq n\|\by_j-\tilde\by\|\|\eta_j-\tilde\eta\|+%\left(\sqrt{\sum_{i=1}^n\epsilon^2_i}\right)
n\|\tilde\by-\boeta_{0n}\|\|\eta_j-\tilde\eta\|+n\|\by_j-\tilde\by\|\|\tilde\eta-\eta_0\|\notag\\
&\qquad\rightarrow 0,~\mbox{as}~\|\by_j-\tilde\by\|\rightarrow 0~\mbox{and}~\|\eta_j-\tilde\eta\|\rightarrow 0,~\mbox{as}~j\rightarrow\infty.\notag
\end{align}
Hence, $\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta(\bx_i)-\eta_0(\bx_i))$ is continuous in $\by_n$ and $\eta$.
Continuity is clearly preserved if the above expression is divided by $\sigma$.

%\begin{align}
%&\Bigg|\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta_1(\bx_i)-\eta_0(\bx_i))-\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta_2(\bx_i)-\eta_0(\bx_i))\Bigg |\label{eq:cont5}\\
%& \ \ \Bigg|\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta_1(\bx_i)-\eta_2(\bx_i))\Bigg |\notag\\
%& \ \ \leq \left(\frac{1}{n}\sum_{i=1}^n\left|\e_i\right|\right)\times\|\eta_1-\eta_2\|,\label{eq:cont6}
%\end{align}
%where, for $i=1,\ldots,n$, $\e_i\stackrel{iid}{\sim}N\left(0,\sigma^2_0\right)$, are almost surely finite. Hence, (\ref{eq:cont6}) implies that, given $\e_1,\ldots,\e_n$, 
%$c_3=\frac{1}{n}\sum_{i=1}^n\left|\e_i\right|$ is a finite quantity. It follows that, if $\|\eta_1-\eta_2\|<\frac{\varepsilon}{c_3}$, then 
%(\ref{eq:cont5}) is less than $\varepsilon$.


Also, the first term of $f(\by_n,\theta)$, given by $\log\left(\frac{\sigma_0}{\sigma}\right)$, is clearly continuous
in $\sigma$. 
%where $\sigma>\xi>0$. That is, for given $\varepsilon>0$, there exists $c_4>0$ such that for $\sigma_1,\sigma_2$, both greater than $\xi$ and satisfying
%$|\sigma_1-\sigma_2|<\frac{\varepsilon}{c_4}$, $\left|\log\sigma_1-\log\sigma_2\right|<\varepsilon$. Hence it follows that for any 
%$\varepsilon>0$, if $c>\max\{c_1,c_2,c_3,c_4\}$, then $\|(\by_{1n},\theta_1)-(\by_{2n},\theta_2)\|<\frac{\varepsilon}{c}$ implies that
%$\left|f(\by_{1n},\theta_1)-f(\by_{1n},\theta_1)\right|<C\varepsilon$, for a finite $C>0$. 
Thus, continuity of $f(\by_n,\theta)$ with respect to $(\by_n,\theta)$ is guaranteed, so that (S1) holds.
Also observe that when the covariates are regarded as random, due to measurability of $\eta_0(\bX)$ assumed in (A4) and continuity of $\eta(\bx)$ in $\bx$.  


\subsection{Verification of (S2) and proof of Lemma \ref{lemma:lemma1} for Gaussian errors}
\label{subsec:S2}
It follows from (\ref{eq:like1}) and (\ref{eq:true_like1}), that
\begin{equation}
\log\frac{f_{\theta_0}(\by_n)}{f_{\theta}(\by_n)}=n\log\left(\frac{\sigma}{\sigma_0}\right)-\frac{1}{2\sigma^2_0}\sum_{i=1}^n(y_i-\eta_0(\bx_i))^2+
\frac{1}{2\sigma^2}\sum_{i=1}^n(y_i-\eta(\bx_i))^2,
\label{eq:logratio1}
\end{equation}
so that
\begin{equation}
\frac{1}{n}E_{\theta_0}\left(\log\frac{f_{\theta_0}(\by_n)}{f_{\theta}(\by_n)}\right)=\log\left(\frac{\sigma}{\sigma_0}\right)-\frac{1}{2}
+\frac{\sigma^2_0}{2\sigma^2}+\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2.
\label{eq:logratio2}
\end{equation}
By (A3), as $n\rightarrow\infty$,
\begin{equation}
\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2\rightarrow E_\bX\left[\eta(\bX)-\eta_0(\bX)\right]^2
=\int_{\mathcal X}\left[\eta(\bX)-\eta_0(\bX)\right]^2dQ.
\label{eq:slln1}
\end{equation}
Hence,
\begin{equation}
\frac{1}{n}E_{\theta_0}\left(\log\frac{f_{\theta_0}(\by_n)}{f_{\theta}(\by_n)}\right)\rightarrow \log\left(\frac{\sigma}{\sigma_0}\right)-\frac{1}{2}
+\frac{\sigma^2_0}{2\sigma^2}+\frac{1}{2\sigma^2}E_\bX\left[\eta(\bX)-\eta_0(\bX)\right]^2,~\mbox{as}~n\rightarrow\infty.
\label{eq:logratio3}
\end{equation}
We let
\begin{equation*}
h(\theta)=\log\left(\frac{\sigma}{\sigma_0}\right)-\frac{1}{2}+\frac{\sigma^2_0}{2\sigma^2}+\frac{1}{2\sigma^2}E_\bX\left[\eta(\bX)-\eta_0(\bX)\right]^2.
%\label{eq:h}
\end{equation*}


\subsection{Verification of (S3) and proof of Theorem \ref{theorem:theorem1} for Gaussian errors}
\label{subsec:S3}


By SLLN, as $n\rightarrow\infty$,
\begin{equation}
\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2\stackrel{a.s.}{\longrightarrow}\sigma^2_0,
\label{eq:slln2}
\end{equation}
where $``\stackrel{a.s.}{\longrightarrow}"$ denotes convergence almost surely.
Also,
\begin{align}
\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta(\bx_i)\right)^2 &=\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2+\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2\notag\\
&\qquad\qquad+\frac{2}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)\left(\eta_0(\bx_i)-\eta(\bx_i)\right).
\label{eq:breakup1}
\end{align}
By (\ref{eq:slln2}) the first term on the right hand side of (\ref{eq:breakup1}) converges almost surely to $\sigma^2_0$. The second term converges to 
$E_{\bX}\left[\eta(\bX)-\eta_0(\bX)\right]^2$ and the
third term converges almost surely to zero by Kolmogorov's SLLN for independent random variables, noting that $y_i-\eta_0(\bx_i)=\e_i$ are independent zero mean random variables
and $\sum_{i=1}^{\infty}i^{-2}Var\left((y_i-\eta_0(\bx_i)(\eta_0(\bx_i)-\eta(\bx_i))\right)=\sigma^2_0\sum_{i=1}^{\infty}i^{-2}\left(\eta_0(\bx_i)-\eta(\bx_i)\right)^2\leq
\sigma^2_0\|\eta-\eta_0\|^2\sum_{i=1}^{\infty}i^{-2}<\infty$. %is independent of $\bX_i$ and hence of $\eta_0(\bx_i)-\eta(\bx_i)$, for $i=1,\ldots,n$.
Hence, letting $n\rightarrow\infty$ in (\ref{eq:R1}), it follows that
\begin{equation}
\frac{1}{n}\log R_n(\theta)\stackrel{a.s.}{\longrightarrow}\log\left(\frac{\sigma_0}{\sigma}\right)+\frac{1}{2}-\frac{\sigma^2_0}{2\sigma^2}
-\frac{1}{2\sigma^2}E_{\bX}\left[\eta(\bX)-\eta_0(\bX)\right]^2=-h(\theta).
\label{eq:R2}
\end{equation}
The above results of course remain the same if the covariates are assumed to be random.

\subsection{Verification of (S4)}
\label{subsec:S4}

Note that $h(\theta)\leq\log\left(\frac{\sigma}{\sigma_0}\right)-\frac{1}{2}+\frac{\sigma^2_0}{2\sigma^2}+\frac{\|\eta-\eta_0\|^2}{2\sigma^2}$, where
$0<\sigma<\infty$ and $0<\|\eta-\eta_0\|<\infty$ with prior probability one. Hence, $h(\theta)<\infty$ with probability one, showing that (S4) holds.
\begin{comment}
By (A5), 
\begin{equation}
\pi\left(\sigma=\infty\right)=0. 
\label{eq:sigma_prior}
\end{equation}
Also, since $\|\eta\|<\infty$ almost surely, and $\|\eta_0\|<\infty$ by (A4), it follows that
\begin{equation}
\pi\left(\|\eta-\eta_0\|=\infty\right)=0.
\label{eq:gp_finite}
\end{equation}
Now, in (\ref{eq:h}) note that $E_\bX\left[\eta(\bX)-\eta_0(\bX)\right]^2\leq \|\eta-\eta_0\|^2$, so that 
\begin{align}
\pi\left(h(\theta)=\infty\right)&\leq\pi\left(\left\{\sigma=\infty\right\}\cup\left\{\|\eta-\eta_0\|=\infty\right\}\right)\notag\\
&\leq\pi\left(\sigma=\infty\right)+\pi\left(\|\eta-\eta_0\|=\infty\right)\notag\\
&=0,~\mbox{due to (\ref{eq:sigma_prior}) and (\ref{eq:gp_finite})}.\notag
\end{align}
Hence, (S4) holds.
\end{comment}

\subsection{Verification of (S5)}
\label{subsec:S5}

\subsubsection{Verification of (S5) (1)}
\label{subsubsec:S5_1}

%Let $\sigma^2_{\mathcal X}=\underset{\bx\in\mathcal X}{\sup}~E\left[\eta(\bx)-\mu(\bx)\right]^2$ and for $j=1,\ldots,d$,
%$\sigma^2_{j,\mathcal X}=\underset{\bx\in\mathcal X}{\sup}~E\left[\eta'_j(\bx)-\mu'_j(\bx)\right]^2$, where $\mu'_j$ stands for the $j$-th partial derivative of $\mu$. 
%Note that, due to compactness of $\mathcal X$,
%these quantities are finite.

%By (A5), there exists $\alpha\in (0,1)$ and $\beta>0$ such that $\alpha\beta>2h(\Theta)$. Now, for any real-valued function $f$ on $\mathcal X$, let us define 
%$\|f\|_0=\underset{\bx\in\mathcal X}{\sup}~f(\bx)$. 
%With this, 
Recall that
\begin{align}
%\mathcal G_n&=\left\{\left(\eta,\sigma\right):\|\eta-\mu\|\leq\sqrt{2\beta\sigma^2_{\mathcal X} n}+E\|\eta-\mu\|,\right.\notag\\
%&\left.\|\eta'_j-\mu'_j\|\leq\sqrt{2\beta\sigma^2_{j,\mathcal X} n}+E\|\eta'_j-\mu'_j\|;j=1,\ldots,d,n^{-\frac{1}{2q}}\leq\sigma\leq\exp\left(\beta n\right)\right\},
\mathcal G_n&=\left\{\left(\eta,\sigma\right):\|\eta\|\leq\exp(\sqrt{\beta n}),\exp(-\sqrt{\beta n})\leq\sigma\leq\exp(\sqrt{\beta n}),
\|\eta'_j\|\leq\exp(\sqrt{\beta n});j=1,\ldots,d\right\}.\notag
%\label{eq:G}
\end{align}
Then $\mathcal G_n\rightarrow\Theta$, as $n\rightarrow\infty$.
%
Now note that
\begin{align}
&\pi(\mathcal G_n)=\pi\left(\|\eta\|\leq\exp(\sqrt{\beta n}),\exp(-\sqrt{\beta n})\leq\sigma\leq\exp(\sqrt{\beta n})\right)\notag\\
%&\ \ -\pi\left(\left\{\|\eta-\mu\|\leq\sqrt{2\beta\sigma^2_{\mathcal X} n}+E\|\eta-\mu\|,\|\eta'_j-\mu'_j\|\leq\sqrt{2\beta\sigma^2_{j,\mathcal X} n}
%+E\|\eta'_j-\mu'_j\|;j=1,\ldots,d\right\}^c\right)\notag\\
&\ \ -\pi\left(\left\{\|\eta'_j\|\leq\exp(\sqrt{\beta n});j=1,\ldots,d\right\}^c\right)\notag\\
%&=\pi\left(n^{-\frac{1}{2q}}\leq\sigma\leq\exp\left(\beta n\right)\right)\notag\\
%&\ \ -\pi\left(\left\{\|\eta-\mu\|>\sqrt{2\beta\sigma^2_{\mathcal X} n}+E\|\eta-\mu\|\right\}\bigcup\left[\bigcup_{j=1}^d\left\{\|\eta'_j-\mu'_j\|>\sqrt{2\beta\sigma^2_{j,\mathcal X} n}
%+E\|\eta'_j-\mu'_j\|\right\}\right]\right)\notag\\
%&=\pi\left(\frac{\|\eta\|}{\sigma}\leq\beta^{\frac{1}{2q}}n^{\frac{1}{2q}},n^{-\frac{1}{2q}}\leq\sigma\leq\beta n\right)\notag\\
%&\ \ -\pi\left(\left\{\|\eta-\mu\|>\sqrt{2\beta\sigma^2_{\mathcal X} n}+E\|\eta-\mu\|\right\}\bigcup\left[\bigcup_{j=1}^d\left\{\|\eta'_j-\mu'_j\|>\sqrt{2\beta\sigma^2_{j,\mathcal X} n}
%+E\|\eta'_j-\mu'_j\|\right\}\right]\right)\notag\\
&=\pi\left(\|\eta\|\leq\exp(\sqrt{\beta n}),\exp(-\sqrt{\beta n})\leq\sigma\leq\exp(\sqrt{\beta n})\right)\notag\\
&\ \ -\pi\left(\bigcup_{j=1}^d\left\{\|\eta'_j\|>\exp(\sqrt{\beta n})\right\}\right)\notag\\
%&\ \ \geq\pi\left(n^{-\frac{1}{2q}}\leq\sigma\leq\exp\left(\beta n\right)\right)-\pi\left(\|\eta-\mu\|>\sqrt{2\beta\sigma^2_{\mathcal X} n}+E\|\eta-\mu\|\right)\notag\\
%&\ \ \  \ -\sum_{j=1}^d\pi\left(\|\eta'_j-\mu'_j\|>\sqrt{2\beta\sigma^2_{j,\mathcal X} n}+E\|\eta'_j-\mu'_j\|\right).
& \geq 1-\pi\left(\|\eta\|>\exp(\sqrt{\beta n})\right)-\pi\left(\left\{\exp(-\sqrt{\beta n})\leq\sigma\leq\exp(\sqrt{\beta n})\right\}^c\right)\notag\\
&\ \ \  \ -\sum_{j=1}^d\pi\left(\|\eta'_j\|>\exp(\sqrt{\beta n})\right)\notag\\
&\geq 1-(c_{\eta}+c_{\sigma}+\sum_{j=1}^dc_{\eta^\prime_j})\exp(-\beta n),
\label{eq:s5_1}
\end{align}
by the Borell-TIS inequality and (A5). 
In other words, (S5) (1) holds.

\subsubsection{Verification of (S5) (2)}
\label{subsubsec:S5_2}

We now show that (S5) (2), namely, convergence in (S3) is uniform in $\theta$ over $\mathcal G_n\setminus I$ holds. First note that $I=\emptyset$ in our case, so that
$\mathcal G_n\setminus I=\mathcal G_n$. 

To proceed further, we show that $\mathcal G_n$ is compact.
Note that $\mathcal G_n=\mathcal G_{n,\eta}\times \mathcal G_{n,\sigma}$, where
\begin{align}
%\mathcal G_{n,\eta}&=\left\{\eta:\|\eta-\mu\|\leq\sqrt{2\beta\sigma^2_{\mathcal X} n}+E\|\eta-\mu\|,\right.\notag\\
\mathcal G_{n,\eta}&=\left\{\eta:\|\eta\|\leq\exp(\sqrt{\beta n}),~\|\eta'_j\|\leq\exp(\sqrt{\beta n});j=1,\ldots,d\right\}\notag
%\label{eq:G_eta}
\end{align}
and
\begin{equation*}
\mathcal G_{n,\sigma}=\left\{\sigma:\exp(-\sqrt{\beta n})\leq\sigma\leq\exp(\sqrt{\beta n})\right\}.
%\label{eq:G_sigma}
\end{equation*}
%Since $\mathcal G_n$ is closed, and closed subsets of compact sets are compact, it is sufficient to prove that $\mathcal G_{n,\eta}\times \mathcal G_{n,\sigma}$ is compact.
Since $\mathcal G_{n,\sigma}$ is compact and products of compact sets is compact, it is enough to prove compactness of $\mathcal G_{n,\eta}$.
We use the Arzela-Ascoli lemma to prove that $\mathcal G_{n,\eta}$ is compact for each $n\geq 1$. 
In other words, $\mathcal G_{n,\eta}$ is compact if and only if it is closed,
bounded and equicontinuous. By boundedness we mean $|\eta(\bx)|<M$ for each $\bx\in\mathcal X$ and for each $\eta\in\mathcal G_{n,\eta}$. Equicontinuity entails
that for any $\epsilon>0$, there exists $\delta>0$ which depends only on $\epsilon$ such that $|\eta(\bx_1)-\eta(\bx_2)|<\epsilon$ whenever $\|\bx_1-\bx_2\|<\delta$,
for all $\eta\in\mathcal G_{n,\eta}$. Closedness and boundedness are obvious from the definition of $\mathcal G_{n,\eta}$. Equicontinuity follows from the fact that
the elements of $\mathcal G_{n,\eta}$ are Lipschitz continuous thanks to boundedness of the partial derivatives. Thus, $\mathcal G_{n,\eta}$, and hence $\mathcal G_n$ is compact.

Since $\mathcal G_n$ is compact for all $n\geq 1$, uniform convergence as required will be proven if we can show that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is 
stochastically equicontinuous almost surely in $\theta\in\mathcal G$ for any 
$\mathcal G\in\left\{\mathcal G_n:n=1,2,\ldots\right\}$ and $\frac{1}{n}\log R_n(\theta)+h(\theta)\rightarrow 0$, almost surely, for all $\theta\in\mathcal G$
(see \ctn{Newey91}, \ctn{Billingsley13}) for the general theory of uniform convergence in compact sets under stochastic equicontinuity). 
Since, in the context of (S3) we have already shown almost sure pointwise convergence of $\frac{1}{n}\log R_n(\theta)$ to $-h(\theta)$, it is enough to verify stochastic
equicontinuity of $\frac{1}{n}\log R_n(\theta)+h(\theta)$ in $\mathcal G\in\left\{\mathcal G_n:n=1,2,\ldots\right\}$.

Stochastic equicontinuity usually follows easily if one can prove that the function concerned is almost surely Lipschitz continuous.
Recall
from (\ref{eq:R1}), (\ref{eq:cont2}), (\ref{eq:breakup2}) and (\ref{eq:cont4}) that if the term $\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta(\bx_i)-\eta_0(\bx_i))$
can be proved Lipschitz continuous in $\eta\in\mathcal G$, then $\frac{1}{n}\log R_n(\theta)$ is Lipschitz for $\eta\in\mathcal G$. Also, if $E_{\bX}\left[\eta(\bX)-\eta_0(\bX)\right]^2$
is Lipschitz in $\eta$, then it would follow from (\ref{eq:h}) that $h(\theta)$ is Lipschitz for $\eta\in\mathcal G$. Since sum of Lipschitz functions is Lipschitz, this would imply
that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is Lipschitz in $\eta\in\mathcal G$. Since the first derivative of $\frac{1}{n}\log R_n(\theta)+h(\theta)$
with respect to $\sigma$ is bounded (as $\sigma$ is bounded in $\mathcal G$), it would then follow that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is Lipschitz for $\theta\in\mathcal G$. 
Hence, to see that $\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta(\bx_i)-\eta_0(\bx_i))$ is almost surely Lipschitz in $\eta\in\mathcal G$, note that for any $\eta_1,\eta_2\in\mathcal G$,
\begin{align}
&\left|\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta_1(\bx_i)-\eta_0(\bx_i))-\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta_2(\bx_i)-\eta_0(\bx_i))\right|\notag\\
&\qquad\qquad\leq\|\eta_1-\eta_2\|\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|.\notag
\end{align}
Hence, $\frac{1}{n}\sum_{i=1}^n(y_i-\eta_0(\bx_i))(\eta(\bx_i)-\eta_0(\bx_i)$ is Lipschitz in $\eta$ and since $\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|\rightarrow
E_{\theta_0}\left|y_1-\eta(\bx_1)\right|\leq E_{\theta_0}\left|y_1-\eta_0(\bx_1)\right|+\left|\eta_0(\bx_1)-\eta(\bx_1)\right|<\infty$ as $n\rightarrow\infty$, stochastic equicontinuity follows.

That $E_{\bX}\left[\eta(\bX)-\eta_0(\bX)\right]^2$ is also Lipschitz in $\mathcal G$ can be seen from the fact that for $\eta_1,\eta_2\in\mathcal G$,
\begin{equation*}
\left|E_{\bX}\left[\eta_1(\bX)-\eta_0(\bX)\right]^2-E_{\bX}\left[\eta_2(\bX)-\eta_0(\bX)\right]^2\right|
\leq\|\eta_1-\eta_2\|\times\left[\|\eta_1\|+\|\eta_2\|+2\|\eta_0\|\right],
\end{equation*}
where $\|\eta_0\|<\kappa_0$ by (A4) and for $j=1,2$, %$\|\eta_j\|\leq\|\eta_j-\mu\|+\|\mu\|\leq\sqrt{2\beta\sigma^2_{\mathcal X}m}+E\|\eta_j-\mu\|+\|\mu\|$, 
$\|\eta_j\|\leq \exp(\sqrt{\beta m})$,
where $\mathcal G=\mathcal G_m$, for $m\geq 1$.

%From the above arguments, it is now clear that all we need to show is the following. For any $\theta\in\mathcal G\in\left\{\mathcal G_n:n=1,2,\ldots\right\}$  
%\begin{equation}
%\sum_{n=1}^{\infty}P\left(\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\delta\right)<\infty,
%\label{eq:uc1}
%\end{equation}
%for any $\delta>0$. 
%From Section \ref{subsec:S1} it follows that $\frac{1}{n}\log R_n(\theta)$ is continuous in $\theta$, and similarly it follows that
%$h(\theta)$ is also continuous in $\theta$. Due to compactness of $\mathcal G_n$ it follows from the extreme value theorem that there exists $\hat\theta\in\mathcal G_n$,
%perhaps depending upon the data, such that $\underset{\theta\in\mathcal G_n}{\sup}~\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|
%=\left|\frac{1}{n}\log R_n(\hat\theta)+h(\hat\theta)\right|$. 
%In what follows, we provide a summable upper bound of the probability
%$P\left(\underset{\theta\in\mathcal G_n}{\sup}~\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\delta\right)
%=P\left(\left|\frac{1}{n}\log R_n(\hat\theta)+h(\hat\theta)\right|>\delta\right)$ by obtaining a summable upper bound of the probability
%$P\left(\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\delta\right)$. %which is independent of any $\theta\in\mathcal G_n$.




%The last step follows because $\frac{\|\eta-\eta_0\|}{\sigma^2}\leq \frac{\|\eta_0\|}{\sigma^2}+\frac{\|\eta\|}{\sigma^2}\leq \frac{\kappa_0}{\xi^2}+\frac{1}{\xi\kappa_1}$, where 
%almost surely, $\frac{\|\eta_0\|}{\sigma^2}\leq\frac{\kappa_0}{\xi^2}$ and $\frac{\|\eta\|}{\sigma^2}\leq\frac{1}{\sigma\kappa_1}\leq \frac{1}{\xi\kappa_1}$ due to (A4) and (A5).

%Gathering the bounds (\ref{eq:s5_7}), (\ref{eq:s5_8}), (\ref{eq:zero_prob}), (\ref{eq:zero_prob2}) and (\ref{eq:s5_9}), all of which are summable with respect to $n$, it follows that 
%(\ref{eq:uc1}) holds, so that (S5) (2) stands verified.

\subsubsection{Verification of (S5) (3)}
\label{subsubsec:S5_3}

We now verify (S5) (3). For our purpose, let us show that $h(\theta)$ is continuous in $\theta$. Continuity will easily follow if we can show that $E_{\bX}\left[\eta(\bX)-\eta_0(\bX)\right]^2$
is continuous in $\eta$. As before, let $\eta_j$ be a sequence of functions converging to $\tilde\eta$ in the sense $\|\eta_j-\tilde\eta\|\rightarrow 0$ as $j\rightarrow\infty$.
Then, since $\left|E_{\bX}\left[\eta_j(\bX)-\eta_0(\bX)\right]^2-E_{\bX}\left[\tilde\eta(\bX)-\eta_0(\bX)\right]^2\right|
\leq \|\eta_j-\tilde\eta\|\left[\|\eta_j-\tilde\eta\|+2\|\tilde\eta-\eta_0\|\right]
\rightarrow 0$ as $j\rightarrow\infty$, continuity follows. Hence, continuity of $h(\theta)$, compactness of $\mathcal G_n$, along with its non-decreasing nature with respect to $n$ implies that 
$h\left(\mathcal G_n\right)\rightarrow h(\Theta)$, as $n\rightarrow\infty$.

\subsection{Verification of (S6) and proof of Theorem \ref{theorem:theorem3} for Gaussian errors}
\label{subsec:S6}



Observe that 
\begin{align}
\frac{1}{n}\log R_n(\theta)+h(\theta)&=\left[\frac{1}{2\sigma^2_0}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{1}{2}\right]
+\left[\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{\sigma^2_0}{2\sigma^2}\right]\notag\\
&\qquad+\left[\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right]\notag\\
&\qquad+\left[\frac{1}{\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)\left(\eta(\bx_i)-\eta_0(\bx_i)\right)\right].
\label{eq:s5_5}
\end{align}
Let $\kappa_1=\kappa-h(\Theta)$. Then it follows from (\ref{eq:s5_5}) that for all $\theta\in\mathcal G$, we have
\begin{align}
&P\left(\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\kappa_1\right)\notag\\
&\leq P\left(\left|\frac{1}{2\sigma^2_0}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{1}{2}\right|>\frac{\kappa_1}{4}\right)
+P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{\sigma^2_0}{2\sigma^2}\right|>\frac{\kappa_1}{4}\right)\notag\\
&\qquad+P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right|>\frac{\kappa_1}{4}\right)\notag\\
&\qquad+P\left(\left|\frac{1}{\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)\left(\eta(\bx_i)-\eta_0(\bx_i)\right)\right|>\frac{\kappa_1}{4}\right).
\label{eq:s5_6}
\end{align}

Note that $\sum_{i=1}^n\left(\frac{y_i-\eta_0(\bx_i)}{\sigma_0}\right)^2=\bz^T_n\bz_n$, %\sim\chi^2_n$, using Markov's inequality similarly as in \ctn{Choi07}, 
where $\bz_n\sim N_n\left(\bzero_n,\bI_n\right)$, the $n$-dimensional normal distribution with mean $\bzero_n=(0,0,\ldots,0)^T$ and covariance matrix $\bI_n$, the identity matrix. 
Using the Hanson-Wright inequality we bound the
first term of the right hand side of (\ref{eq:s5_6}) as follows:
\begin{align}
&P\left(\left|\frac{1}{2\sigma^2_0}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{1}{2}\right|>\frac{\kappa_1}{4}\right)\notag\\
&\qquad=P\left(\left|\bz^T_n\bz_n-n\right|>\frac{n\kappa_1}{2}\right)\notag\\
&\qquad\leq 2\exp\left(-n\min\left\{\frac{\kappa^2_1}{16c_0},\frac{\kappa_1}{4c_0}\right\}\right),
%&=P\left(\sum_{i=1}^n\left(\frac{y_i-\eta_0(\bx_i)}{\sigma_0}\right)^2>n\left(1+\frac{\kappa_1}{2}\right)\right)
%+P\left(\sum_{i=1}^n\left(\frac{y_i-\eta_0(\bx_i)}{\sigma_0}\right)^2<n\left(1-\frac{\kappa_1}{2}\right)\right)\notag\\
%&\leq\exp\left\{-n\left(\frac{\kappa^2_1}{16}-\frac{\kappa^3_1}{48}\right)\right\}+\exp\left\{-n\left(\frac{\kappa^2_1}{16}\right)\right\}.
\label{eq:s5_7}
\end{align}
where $c_0>0$ is a constant.
It follows from (\ref{eq:s5_7}) that
\begin{equation}
\int_{\mathcal S^c}P\left(\left|\frac{1}{2\sigma^2_0}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{1}{2}\right|>\frac{\kappa_1}{4}\right)d\pi(\theta)
\leq 2\exp\left(-n\min\left\{\frac{\kappa^2_1}{16c_0},\frac{\kappa_1}{4c_0}\right\}\right).
\label{eq:s5_7_int}
\end{equation}

In almost the same way as in (\ref{eq:s5_7}), the second term of the right hand side of (\ref{eq:s5_6}) can be bounded as:
\begin{align}
&P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{\sigma^2_0}{2\sigma^2}\right|>\frac{\kappa_1}{4}\right)\notag\\
&\qquad=P\left(\left|\bz^T_n\bz_n-n\right|>\frac{n\kappa_1\sigma^2}{2\sigma^2_0}\right)\notag\\
&\qquad\leq 2\exp\left(-n\min\left\{\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0},\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right\}\right).
%&=P\left(\left|\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-1\right|>\frac{\kappa_1\sigma^2}{2\sigma^2_0}\right)\notag\\
%&\leq P\left(\left|\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-1\right|>\frac{\delta\xi^2}{2\sigma^2_0}\right)\notag\\
%&=P\left(\sum_{i=1}^n\left(\frac{y_i-\eta_0(\bx_i)}{\sigma_0}\right)^2>n\left(1+\frac{\kappa_1\sigma^2}{2\sigma^2_0}\right)\right)
%+P\left(\sum_{i=1}^n\left(\frac{y_i-\eta_0(\bx_i)}{\sigma_0}\right)^2<n\left(1-\frac{\kappa_1\sigma^2}{2\sigma^2_0}\right)\right)\notag\\
%&\leq\exp\left\{-n\left(\frac{\kappa^2_1\sigma^4}{16\sigma^4_0}-\frac{\kappa^3_1\sigma^6}{48\sigma^6_0}\right)\right\}
%+\exp\left\{-n\left(\frac{\kappa^2_1\sigma^4}{16\sigma^4_0}\right)\right\}.
\label{eq:s5_8}
\end{align}
Now
\begin{align}
&\int_{\mathcal S^c}P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)^2-\frac{\sigma^2_0}{2\sigma^2}\right|>\frac{\kappa_1}{4}\right)d\pi(\theta)\notag\\
&\leq \int_{\mathcal G_n}2\exp\left(-n\min\left\{\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0},\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right\}\right)\pi(\sigma^2)d\sigma^2\notag\\
&\qquad+\int_{\mathcal G^c_n}2\exp\left(-n\min\left\{\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0},\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right\}\right)\pi(\theta)d\theta\notag\\
&\leq \int_{\mathcal G_n}2\exp\left(-n\min\left\{\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0},\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right\}\right)\pi(\sigma^2)d\sigma^2
+2\pi(\mathcal G^c_n)\notag\\
&\leq \int_{\mathcal G_n\cap\left\{\frac{\kappa_1\sigma^2}{4\sigma^2_0}\leq 1\right\}}2\exp\left(-n\min\left\{\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0},\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right\}\right)\pi(\sigma^2)d\sigma^2\notag\\
&\qquad+\int_{\mathcal G_n\cap\left\{\frac{\kappa_1\sigma^2}{4\sigma^2_0}> 1\right\}}2\exp\left(-n\min\left\{\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0},\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right\}\right)\pi(\sigma^2)d\sigma^2+2\pi(\mathcal G^c_n)\notag\\
&=\int_{\mathcal G_n\cap\left\{\frac{\kappa_1\sigma^2}{4\sigma^2_0}\leq 1\right\}}2\exp\left(-n\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0}\right)\pi(\sigma^2)d\sigma^2\notag\\
&\qquad+\int_{\mathcal G_n\cap\left\{\frac{\kappa_1\sigma^2}{4\sigma^2_0}> 1\right\}}2\exp\left(-n\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right)\pi(\sigma^2)d\sigma^2+2\pi(\mathcal G^c_n)\notag\\
&\leq\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}2\exp\left(-n\frac{\kappa^2_1\sigma^4}{16c_0\sigma^4_0}\right)\pi(\sigma^2)d\sigma^2\notag\\
&\qquad+\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}2\exp\left(-n\frac{\kappa_1\sigma^2}{4c_0\sigma^2_0}\right)\pi(\sigma^2)d\sigma^2+2\pi(\mathcal G^c_n)\notag\\
&=\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}2\exp\left(-n\frac{\kappa^2_1u^{-2}}{16c_0\sigma^4_0}\right)\pi(u^{-1})u^{-2}du\notag\\
&\qquad+\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}2\exp\left(-n\frac{\kappa_1u^{-1}}{4c_0\sigma^2_0}\right)\pi(u^{-1})u^{-2}du+2\pi(\mathcal G^c_n).
\label{eq:s5_8_int}
\end{align}

Let us first consider the first term of (\ref{eq:s5_8_int}). Note that the prior $\pi\left(u^{-1}\right)u^{-2}$ is such that large values of $u$ receive
small probabilities. Hence, if this prior is replaced by an appropriate function which has a thicker tail than the prior, then the resultant integral provides an upper bound
for the first term of (\ref{eq:s5_8_int}). We consider a function 
%Note that for priors with very thick tails the above method with $\tilde\pi(u)$ of the above form need not be suitable. In such cases we let 
$\tilde\pi(u)$ which is of mixture form depending upon $n$, that is, 
we let $\tilde\pi_n(u)=c_3\sum_{r=1}^{M_n}\psi^{\zeta_{rn}}_{rn}\exp(-\psi_{rn} u^2)u^{2(\zeta_{rn}-1)}$, 
where %$B_n=\left[\exp\left(-2\sqrt{\beta n}\right),\exp\left(2\sqrt{\beta n}\right)\right]$, 
$M_n\leq\exp(\sqrt{\beta n})$ is the number of mixture components, $c_3>0$,  
for $r=1,\ldots,M_n$, $\frac{1}{2}<\zeta_{rn}\leq c_4n^q$, for $0<q<1/2$ and $n\geq 1$, where $c_4>0$, and $0<\psi_1\leq\psi_{rn}<c_5<\infty$, for all $r$ and $n$. 
In this case, with $C_1=\frac{1}{16c_0\sigma^4_0}$,
\begin{align}
& \int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}\exp\left(-C_1\kappa^2_1nu^{-2}\right)\pi(u^{-1})u^{-2}du\notag\\
%&\leq C_2\int_{\exp(-2\sqrt{\alpha T})-\sigma^{-2}_0}^{\exp(2\sqrt{\alpha T})-\sigma^{-2}_0}\exp\left[-\left(C_1mu^{-2}+\frac{u^2}{2\sigma^2_1}\right)\right]u^{-2}du.
&\leq c_3\sum_{r=1}^{M_n}\psi^{\zeta_{rn}}_{rn}
\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}\exp\left[-\left(C_1\kappa^2_1nu^{-2}+\psi_{rn}u^2\right)\right]\left(u^2\right)^{\zeta_{rn}-1}du.
\label{eq:term1_bound3_1}
\end{align}
Now the $r$-th integrand of (\ref{eq:term1_bound3_1}) is minimized at %$\tilde u=\sigma^2_1\left(\sqrt{1+\frac{2C_1m}{\sigma^2_1}}-1\right)$, 
$\tilde u^2_{rn}= \frac{\zeta_{rn}-1+\sqrt{(\zeta_{rn}-1)^2+4C_1\psi_{rn}\kappa^2_1 n}}{2\psi_{rn}}$, so that for sufficiently large $n$, 
$c_1\kappa_1\sqrt{\frac{n}{\psi_{rn}}}\leq\tilde u^2_{rn}\leq \tilde c_1\kappa_1\sqrt{\frac{n}{\psi_{rn}}}$, for some positive constants $c_1$ and $\tilde c_1$. 
Now, for sufficiently large $n$, we have $\frac{\tilde u^2_{rn}}{\log\tilde u^2_{rn}}\geq\frac{\zeta_{rn}-1}{\psi_{rn}(1-c_2)}$, for $0<c_2<1$.
Hence, for sufficiently large $n$, $C_1\kappa^2_1n\tilde u^{-2}_{rn}+\psi_{rn}\tilde u^2_{rn}-(\zeta_{rn}-1)\log(\tilde u^2_{rn})\geq c_2\psi_1\tilde u^2_{rn}
\geq C_2\kappa_1\sqrt{\psi_{rn} n}$ for some 
positive constant $C_2$. From these and (\ref{eq:term1_bound3_1}) it follows that
\begin{align}
&\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}2\exp\left(-n\frac{\kappa^2_1u^{-2}}{16c_0\sigma^4_0}\right)\pi(u^{-1})u^{-2}du\notag\\
&=c_3\sum_{r=1}^{M_n}\psi^{\zeta_{rn}}_{rn}
\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}\exp\left[-\left(C_1\kappa^2_1nu^{-2}+\psi_1u^2\right)\right]\left(u^2\right)^{\zeta_{rn}-1}du\notag\\
&\leq c_3M_n\exp\left[-\left(C_2\kappa_1\sqrt{n\psi_1}-2\sqrt{\beta n}-\tilde c_5 n^q\right)\right]\notag\\
&\leq c_3\exp\left[-\left(C_2\kappa_1\sqrt{n\psi_1}-3\sqrt{\beta n}-\tilde c_5 n^q\right)\right].
\label{eq:term1_bound3_2}
\end{align}
for some constant $\tilde c_5$. 
Since $\kappa_1$ is as large as desired, $C_2\kappa_1\sqrt{n\psi_1}-3\sqrt{\beta n}-\tilde c_5 n^q>0$ for large enough $n$.

For the second term of (\ref{eq:s5_8_int}), we consider $\tilde\pi_n(u)=c_3\sum_{r=1}^{M_n}\psi^{\zeta_{rn}}_{rn}\exp(-\psi_{rn} u)u^{(\zeta_{rn}-1)}$, with
$M_n\leq\exp(\sqrt{\beta n})$ is the number of mixture components, $c_3>0$, for $r=1,\ldots,M_n$, $0<\zeta_{rn}\leq c_4n^q$, for $0<q<1/2$ and $n\geq 1$, 
where $c_4>0$, and $0<\psi_1\leq\psi_{rn}<c_5<\infty$, for all $r$ and $n$. Thus, the only difference here with the previous definition of $\tilde\pi_n(u)$
is that here $\zeta_{rn}>0$ instead of $\zeta_{rn}>\frac{1}{2}$, which is due to the fact that here $u^2$ is replaced with $u$. In the same way as in (\ref{eq:term1_bound3_2}), it then
follows that
\begin{equation}
\int_{\exp(-2\sqrt{\beta n})}^{\exp(2\sqrt{\beta n})}2\exp\left(-n\frac{\kappa_1u^{-1}}{4c_0\sigma^2_0}\right)\pi(u^{-1})u^{-2}du
\leq c_3\exp\left[-\left(C_2\sqrt{\kappa_1n\psi_1}-3\sqrt{\beta n}-\tilde c_5 n^q\right)\right].
\label{eq:term1_bound3_3}
\end{equation}
Again, $C_2\sqrt{\kappa_1n\psi_1}-3\sqrt{\beta n}-\tilde c_5 n^q>0$ for sufficiently large $n$.


%The third term of the right hand side of (\ref{eq:s5_6}) is the probability of a deterministic quantity with respect to the distribution of $\by_n$, and is zero for large enough 
%$n$ due to (\ref{eq:slln1}). In other words, there exists $n_0\geq 1$ such that for $n\geq n_0$,
%\begin{equation}
%P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
%-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right|>\frac{\kappa_1}{4}\right)=0.
%\label{eq:zero_prob}
%\end{equation}
%In the case of random covariates $\bX$, it can be proved in the same way as (\ref{eq:bound_reference}), using the fact that 
%$\underset{\bx\in\mathcal X}{\sup}~\left(\eta(\bx)-\eta_0(\bx)\right)^2 \leq \|\eta-\eta_0\|^2$, that 
%\begin{equation}
%P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
%-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right|>\frac{\delta}{4}\right)
%=O\left(n^{-3}\right).
%\label{eq:zero_prob2}
%\end{equation}
For the third term, let us first consider the case of random covariates $\bX$. Here observe that by Hoeffding's inequality (\ctn{Hoeffding63}),
\begin{align}
&P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right|>\frac{\kappa_1}{4}\right)\notag\\
&\qquad\leq \exp\left\{-\frac{n^2\kappa^2_1\sigma^4}{144n\|\eta-\eta_0\|^2}\right\}=\exp\left\{-\frac{n\kappa^2_1\sigma^4}{144\|\eta-\eta_0\|^2}\right\},
\label{eq:zero_prob2}
\end{align}
where $\|\eta-\eta_0\|$ is clearly the upper bound of $|\eta(\cdot)-\eta_0(\cdot)|$. Such an upper bound is finite since $\mathcal X$ is compact, $\eta(\cdot)$ is continuous on $\mathcal X$,
and $\|\eta_0\|<\infty$. The same inequality holds when the covariates are non-random; here we can view $\varphi(\bx_i)$; $i=1,\ldots,n$, as a set of independent realizations
from some independent stochastic process.

It follows that
\begin{align}
&\int_{\mathcal S^c}P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right|>\frac{\kappa_1}{4}\right)d\pi(\theta)\notag\\
&\leq\int_{\mathcal G_n}\exp\left\{-\frac{n\kappa^2_1\sigma^4}{144\|\eta-\eta_0\|^2}\right\}d\pi(\theta)+\pi(\mathcal G^c_n)\notag\\
&=\int_{\|\eta\|\leq\exp(\sqrt{\beta n})}\|\eta-\eta_0\|\left[\int_{\|\eta-\eta_0\|\exp(-2\sqrt{\beta n})}^{\|\eta-\eta_0\|\exp(2\sqrt{\beta n})}
\exp\left(-\frac{n\kappa^2_1u^{-2}}{144}\right)\pi\left(\frac{\|\eta-\eta_0\|}{u}\right)u^{-2}du\right]\pi\left(\|\eta\|\right)d\|\eta\|\notag\\
&\qquad+\pi(\mathcal G^c_n).
\label{eq:zero_prob3}
\end{align}

Since $\pi\left(\sigma^2>\exp(2\sqrt{\beta n})\right)\leq \exp(-\beta n)$, it is evident that small values of $u$ receive little mass with respect to %much the mass of 
$\pi\left(\frac{\|\eta-\eta_0\|}{u}\right)u^{-2}$. %is concentrated around zero, where the function
%However, the function $\exp\left(-\frac{n\kappa^2_1u^{-2}}{144}\right)$ is large for small values of $u$, so that the first term of (\ref{eq:zero_prob3}) is relatively small.
%$\exp\left(-C_{11}nu^{-2}\right)$ is small. 
%To give greater weight to the function, we can replace 
To obtain an upper bound to the first term of (\ref{eq:zero_prob3}), as before we replace
$\pi\left(\frac{\|\eta-\eta_0\|}{u}\right)u^{-2}$
with a thick-tailed mixture function of the form $\tilde\pi_{\eta,n}(u)
=c_3\sum_{r=1}^{M_n}\|\eta-\eta_0\|^{\zeta_{rn}}\psi^{\zeta_{rn}}_{rn}\exp\left(-u^2\psi_{rn}\|\eta-\eta_0\|\right)\left(u^2\right)^{(\zeta_{rn}-1)}$, 
for positive constants $0<\psi_2\leq\psi_{rn}<c_5<\infty$ and $\frac{1}{2}<\zeta_{rn}<c_4n^q$. 
%Here $$B_{n,\rho^2}=\left[\rho^2\exp(-2\sqrt{\alpha n})-\frac{\rho^2_0}{\sigma^2_0}, \rho^2\exp(2\sqrt{\alpha n})-\frac{\rho^2_0}{\sigma^2_0}\right].$$
Note that for large values of $\|\eta-\eta_0\|$, $\pi\left(\frac{\|\eta-\eta_0\|}{u}\right)u^{-2}$ is small. %large, and small for large $\rho^2$.
This property is broadly inherited by $\tilde\pi_{\eta,n}$, while the tuning parameters $\psi_{rn}$ and $\zeta_{rn}$ can be adjusted to give prior weight to regions far away from zero.
However in $\tilde\pi_{\eta,n}(u)$, note that for $\|\eta-\eta_0\|\geq 1$, $\exp\left(-u^2\psi_{rn}\|\eta-\eta_0\|\right)\leq \exp\left(-u^2\psi_{rn}\right)$, while for $\|\eta-\eta_0\|<1$, 
%the integral of the first term of (\ref{eq:zero_prob3}) must be
%small thanks to multiplication of the range of the integral and the integral itself with $\|\eta-\eta_0\|$. 
the domain of the function $\pi\left(\frac{\|\eta-\eta_0\|}{u}\right)$ is dominated by $u^{-1}$, which is independent of $\eta$.
Hence, for small $\|\eta-\eta_0\|$ 
it suffices to consider a mixture of $\psi^{\zeta_{rn}}_{rn}\exp\left(-u^2\psi_{rn}\right)\left(u^2\right)^{(\zeta_{rn}-1)}$.
%(or a mixture of $M_T$ such terms with different values of $\tilde\psi_6$ and $\tilde\zeta_6$ depending upon $T$) instead of $\exp\left(-u^2\psi_6\rho^2\right)$.
In other words, for all values of $\|\eta-\eta_0\|$, it is sufficient to consider 
$\tilde\pi_n(u)=c_3\sum_{r=1}^{M_n}\psi^{\zeta_{rn}}_{rn}\exp\left(-u^2\psi_{rn}\right)\left(u^2\right)^{(\zeta_{rn}-1)}$.
Hence, up to some positive constant,
\begin{align}
&\int_{\|\eta-\eta_0\|\exp(-2\sqrt{\beta n})}^{\|\eta-\eta_0\|\exp(2\sqrt{\beta n})}\exp\left(-\frac{\kappa^2_1nu^{-2}}{144}\right)
\pi\left(\frac{\|\eta-\eta_0\|}{u}\right)u^{-2}du\notag\\
&\leq \sum_{r=1}^{M_n}\psi^{\zeta_{rn}}_{rn}
\int_{\|\eta-\eta_0\|\exp(-2\sqrt{\beta n})}^{\|\eta-\eta_0\|\exp(2\sqrt{\beta n})}
\exp\left[-\left(\frac{\kappa^2_1nu^{-2}}{144}+\psi_{rn}u^2-(\zeta_{rn}-1)\log u^2\right)\right]du.
\label{eq:root1}
\end{align}
The term within the parenthesis in the exponent of (\ref{eq:root1}) is minimized at $\tilde u^2_{rn}=\frac{\zeta_{rn}-1+\sqrt{(\zeta_{rn}-1)^2+\frac{\psi_{rn}\kappa^2_1n}{36}}}{2\psi_{rn}}$.
Note that $\tilde C_{01}\kappa_1\sqrt{\frac{n}{\psi_{rn}}}\leq\tilde u^2_{rn}\leq\tilde C_{11}\kappa_1\sqrt{\frac{n}{\psi_{rn}}}$, for large enough $n$, for positive constants
$\tilde C_{01}$ and $\tilde C_{11}$. Hence, for large $n$, the 
term within the parenthesis in the exponent of (\ref{eq:root1}) exceeds $\psi_{rn}\tilde u^2\geq \tilde C_{02}\times\kappa_1\sqrt{\psi_{rn} n}$, for $\tilde C_{02}>0$.
Thus, (\ref{eq:root1}) is bounded above by a constant times $\|\eta-\eta_0\|\exp\left(-\tilde C_{02}\times\kappa_1\sqrt{\psi_2 n}+3\sqrt{\beta n}+\tilde c_5 n^q\right)$.
Hence, %the first term of (\ref{eq:zero_prob3}) is bounded above by 
\begin{align}
&\int_{\mathcal S^c}P\left(\left|\frac{1}{2\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
-\frac{1}{2\sigma^2}E_{\bX}\left(\eta(\bX)-\eta_0(\bX)\right)^2\right|>\frac{\kappa_1}{4}\right)d\pi(\theta)\notag\\
&\qquad\leq 4\exp\left(-\tilde C_{02}\times\kappa_1\sqrt{\psi_2 n}+5\sqrt{\beta n}+\tilde c_5 n^q\right)+\pi\left(\mathcal G^c_n\right).
\label{eq:zero_prob4}
\end{align}
Since $\kappa_1$ is as large as desired, the exponent is negative.

For the fourth term, note that 
$$
Z_n=\frac{1}{n}\sum_{i=1}^n\left(\frac{y_i-\eta_0(\bx_i)}{\sigma_0}\right)\left(\eta(\bx_i)-\eta_0(\bx_i)\right) 
\sim N\left(0,\frac{1}{n^2}\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)\right).$$
Then since
$$\sum_{i=1}^n\left(\eta(\bx_i)-\eta_0(\bx_i)\right)^2
\leq n\left(\underset{\bx\in\mathcal X}{\sup}~|\eta(\bx)-\eta_0(\bx)|\right)^2=n\|\eta-\eta_0\|^2,$$
\begin{align}
&P\left(\left|\frac{1}{\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)\left(\eta(\bx_i)-\eta_0(\bx_i)\right)\right|>\frac{\kappa_1}{4}\right)
= P\left(\left|Z_n\right|>\frac{\kappa_1\sigma^2}{4\sigma_0}\right)\notag\\
&\ \ \leq 2\exp\left(-\frac{n\kappa^2_1\sigma^4}{32\sigma^2_0\|\eta-\eta_0\|^2}\right).
%&\ \ \leq E\left(Z^6_n\right)\left(\frac{4\sigma_0}{\delta\sigma^2}\right)^6
%=15n^{-6}\left(\frac{4\sigma_0}{\delta\sigma^2}\right)^6\left[\sum_{i=1}^n(\eta(\bx_i)-\eta_0(\bx_i))^2\right]^3\notag\\
%&\ \ \leq 15n^{-3}\left(\frac{4\sigma_0}{\delta}\right)^6\left(\frac{\|\eta-\eta_0\|}{\sigma^2}\right)^6.
%%&\ \ \leq 15n^{-3}\left(\frac{4\sigma_0}{\delta}\right)^6\left(\frac{\kappa_0}{\xi^2}+\frac{1}{\xi\kappa_1}\right)^6. 
\label{eq:s5_9}
\end{align}
Hence, in the same way as (\ref{eq:zero_prob4}), we obtain
\begin{align}
&\int_{\mathcal S^c}P\left(\left|\frac{1}{\sigma^2}\times\frac{1}{n}\sum_{i=1}^n\left(y_i-\eta_0(\bx_i)\right)
\left(\eta(\bx_i)-\eta_0(\bx_i)\right)\right|>\frac{\kappa_1}{4}\right)d\pi(\theta)\notag\\
&\leq \int_{\mathcal G_n}2\exp\left(-\frac{n\kappa^2_1\sigma^4}{32\sigma^2_0\|\eta-\eta_0\|^2}\right)d\pi(\theta)+2\pi\left(\mathcal G^c_n\right)\notag\\
&\leq 4\exp\left(-\tilde C_{03}\times\kappa_1\sqrt{\psi_3 n}+5\sqrt{\beta n}+\tilde c_5 n^q\right)+2\pi\left(\mathcal G^c_n\right),
\label{eq:zero_prob5}
\end{align}
for some positive constant $\tilde C_{03}$. As in (\ref{eq:zero_prob3}), the exponent is negative.

Combining (\ref{eq:s5_6}), (\ref{eq:s5_7_int}), (\ref{eq:s5_8_int}), (\ref{eq:term1_bound3_2}), (\ref{eq:term1_bound3_3}), (\ref{eq:zero_prob3}), (\ref{eq:zero_prob4}), (\ref{eq:zero_prob5}),
and noting that $\sum_{n=1}^{\infty}\pi\left(\mathcal G^c_n\right)<\sum_{n=1}^{\infty}\alpha\exp\left(-\beta n\right)<\infty$, we obtain
\begin{equation*}
\int_{\mathcal S^c}P\left(\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\kappa_1\right)d\pi(\theta)<\infty.
\end{equation*}

\subsection{Verification of (S7)}
\label{subsec:S7}
For any set $A$ such that $\pi(A)>0$, $\mathcal G_n\cap A\uparrow A$. It follows from this and continuity of $h$ that $h\left(\mathcal G_n\cap A\right)\downarrow h\left(A\right)$ as
$n\rightarrow\infty$, so that (S7) holds.

%Thus, all the assumptions (S1)--(S7) are satisfied, showing that Theorems \ref{theorem:shalizi1} and \ref{theorem:shalizi2} hold.
%Formally, we have the following theorem.
%\begin{theorem}
%\label{theorem:gp1}
%Assume the Gaussian process model given by (\ref{eq:model1}), (\ref{eq:model2}), (\ref{eq:gp1}) and (\ref{eq:prior_sigma}). Then under the conditions (A1) -- (A5),
%(\ref{eq:supp_post_conv1}) holds. 
%Also, for any measurable set $A$ with $\pi(A)>0$, if $\beta>2h(A)$, where $h$ is given by (\ref{eq:h}), or if $A\subset\cap_{k=n}^{\infty}\mathcal G_k$ for some $n$, 
%where $\mathcal G_k$ is given by (\ref{eq:G}), then
%(\ref{eq:post_conv2}) holds.
%\end{theorem}


\section{Verification of Shalizi's conditions for Gaussian process regression with double exponential error distribution}
\label{sec:de}

%We now assume the same set-up as (\ref{eq:model1}), (\ref{eq:gp1}) and (\ref{eq:prior_sigma}), but assume that $\epsilon_i\stackrel{iid}{\sim}DE(0,\sigma)$, where
%$DE(0,\sigma)$ stands for the double exponential distribution with median $0$ and scale parameter $\sigma$ with density 
%\begin{equation}
%f(\epsilon)=\frac{1}{2\sigma}\exp\left(-\frac{|\epsilon|}{\sigma}\right);~\epsilon\in\mathbb R.
%\label{eq:de1}
%\end{equation}

%\begin{align}
%y_i&=\eta(\bx_i)+\epsilon_i;~i=1,\ldots,n;\label{eq:model1}\\
%\epsilon_i &\stackrel{iid}{\sim}N\left(0,\sigma^2\right);\label{eq:model2}\\
%\eta(\cdot) &\sim GP\left(\mu(\cdot),c(\cdot,\cdot)\right);\label{eq:gp1}\\
%\sigma &\sim\pi_{\sigma}(\cdot).
%\label{eq:prior_sigma}
%\end{align}

\subsection{Verification of (S1)}
\label{subsec:S1_de}
In this case,
\begin{equation}
\frac{1}{n}\log R_n(\theta)=\log\left(\frac{\sigma_0}{\sigma}\right)+\frac{1}{\sigma_0}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta_0(\bx_i)\right)|
-\frac{1}{\sigma}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|.
\label{eq:R_de}
\end{equation}
%We show that the right hand side of (\ref{eq:R1}), which we denote as $f(\by_n,\theta)$, is continuous in $(\by_n,\theta)$, which is sufficient to confirm measurability of $R_n(\theta)$.
%Let $\|(\by_n,\theta)\|=\|\by_n\|+\|\theta\|$, where $\|\by_n\|$ is the Euclidean norm and $\|\theta\|=\|\eta\|+|\sigma|$, with
%$\|\eta\|=\underset{\bx\in\mathcal X}{\sup}~|\eta(\bx)|$. Since $\mathcal X$ is compact and $\eta$ is almost surely continuous, it follows that $\|\eta\|<\infty$ almost surely.
%
%Consider $\by_{1n}=(y_{11},y_{12},\ldots,y_{1n})^T$, $\by_{2n}=(y_{21},y_{22},\ldots,y_{2n})^T$, $\theta_1$ and $\theta_2$ 
%such that, given $\varepsilon>0$, $\|(\by_{1n},\theta_1)-(\by_{2n},\theta_2)\|<\frac{\varepsilon}{c}$, for some finite $c>0$.
%Letting $\boeta_{0n}=(\eta_0(\bx_1),\ldots,\eta_0(\bx_n))^T$, observe that
As before, note that
\begin{align}
&\Bigg|\frac{1}{n}\sum_{i=1}^n\left|y_{1i}-\eta_0(\bx_i)\right|-\frac{1}{n}\sum_{i=1}^n\left|y_{2i}-\eta_0(\bx_i)\right|\Bigg |\notag\\
&\leq\frac{1}{n}\sum_{i=1}^n\Bigg |\left|y_{1i}-\eta_0(\bx_i)\right|-\left|y_{2i}-\eta_0(\bx_i)\right|\Bigg |\notag\\
&\leq\frac{1}{n}\sum_{i=1}^n|y_{1i}-y_{2i}|\notag\\
&\leq n^{-\frac{1}{2}}\sqrt{\sum_{i=1}^n(y_{1i}-y_{2i})^2}\notag\\
&=n^{-\frac{1}{2}}\|\by_{1n}-\by_{2n}\|,\notag
%&\ \ \leq\|\by_{1n}-\by_{2n}\|\times\left(\frac{\|\by_{1n}-\boeta_{0n}\|}{n}+\frac{\|\by_{2n}-\boeta_{0n}\|}{n}\right).
%\label{eq:cont3}
\end{align}
from which Lipschitz continuity follows.
Similarly, 
\begin{align}
&\Bigg|\frac{1}{n}\sum_{i=1}^n\left|y_{1i}-\eta_1(\bx_i)\right|-\frac{1}{n}\sum_{i=1}^n\left|y_{2i}-\eta_2(\bx_i)\right|\Bigg |\notag\\ 
&\leq\frac{1}{n}\sum_{i=1}^n\left|y_{1i}-\eta_1(\bx_i)-y_{2i}+\eta_2(\bx_i)\right|\notag\\
&\leq\frac{1}{n}\sum_{i=1}^n\left[\left|y_{1i}-y_{2i}\right|+\left|\eta_1(\bx_i)-\eta_2(\bx_i)\right|\right]\notag\\
&\leq n^{-\frac{1}{2}}\|\by_1-\by_2\|+\|\eta_1-\eta_2\|,
\label{eq:lipcont_de}
\end{align}
which implies continuity of $\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|$ with respect to $\by$ and $\eta$.
In other words, (\ref{eq:R2}) is continuous and hence measurable, as before. Measurability, when the covariates are considered random, also follows as before,
using measurability of $\eta_0(\bX)$ as assumed in (A4).

\subsection{Verification of (S2) and proof of Lemma \ref{lemma:lemma1} for double-exponential errors}
\label{subsec:S2_de}
Now note that if $\epsilon_i=y_i-\eta_0(\bx_i)$ has the double exponential density of the form 
\begin{equation*}
f(\epsilon)=\frac{1}{2\sigma}\exp\left(-\frac{|\epsilon|}{\sigma}\right);~\epsilon\in\mathbb R.
%\label{eq:de1}
\end{equation*}
with $\sigma$ replaced with $\sigma_0$, then
\begin{align}
&E_{\theta_0}\left|y_i-\eta_0(\bx_i)\right|=\sigma_0;\label{eq:de_exp1}\\ 
&E_{\theta_0}\left|y_i-\eta(\bx_i)\right|=E_{\theta_0}\left|(y_i-\eta_0(\bx_i))+(\eta_0(\bx_i)-\eta(\bx_i))\right|\notag\\
&\qquad\qquad\qquad\quad=|\eta_0(\bx_i)-\eta(\bx_i)|+\sigma_0\exp\left(-\frac{|\eta_0(\bx_i)-\eta(\bx_i)|}{\sigma_0}\right).
\label{eq:de_exp2}
\end{align}
It follows from (\ref{eq:de_exp1}), (\ref{eq:de_exp2}) and (A3), that
\begin{align}
&\frac{1}{n}\sum_{i=1}^nE_{\theta_0}\left|y_i-\eta_0(\bx_i)\right|=\sigma_0;\label{eq:de_exp3}\\
&\frac{1}{n}\sum_{i=1}^nE_{\theta_0}\left|y_i-\eta(\bx_i)\right|=
\frac{1}{n}\sum_{i=1}^n\left[|\eta(\bx_i)-\eta_0(\bx_i)|+\sigma_0\exp\left(-\frac{|\eta(\bx_i)-\eta_0(\bx_i)|}{\sigma_0}\right)\right]\notag\\
&\ \ \rightarrow E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|+\sigma_0E_{\bX}\left[\exp\left(-\frac{|\eta(\bX)-\eta_0(\bX)|}{\sigma_0}\right)\right],
~\mbox{as}~n\rightarrow\infty.\label{eq:de_exp4}
\end{align}
Using (\ref{eq:de_exp3}) and (\ref{eq:de_exp4}) we see that as $n\rightarrow\infty$,
\begin{align}
&\frac{1}{n}E_{\theta_0}\left[\log R_n(\theta)\right]=\log\left(\frac{\sigma_0}{\sigma}\right)
+\frac{1}{\sigma_0}\times\frac{1}{n}\sum_{i=1}^nE_{\theta_0}\left|y_i-\eta_0(\bx_i)\right|
-\frac{1}{\sigma}\times\frac{1}{n}\sum_{i=1}^nE_{\theta_0}\left|y_i-\eta(\bx_i)\right|\notag\\
&\rightarrow\log\left(\frac{\sigma_0}{\sigma}\right)+1-\frac{1}{\sigma}E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|
-\frac{\sigma_0}{\sigma}E_{\bX}\left[\exp\left(-\frac{|\eta(\bX)-\eta_0(\bX)|}{\sigma_0}\right)\right],\notag\\
&\ \ =-h(\theta),
\label{eq:R_de2}
\end{align}
where
\begin{equation*}
h(\theta)=\log\left(\frac{\sigma}{\sigma_0}\right)-1+\frac{1}{\sigma}E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|
+\frac{\sigma_0}{\sigma}E_{\bX}\left[\exp\left(-\frac{|\eta(\bX)-\eta_0(\bX)|}{\sigma_0}\right)\right].
%\label{eq:h_de}
\end{equation*}
As in the case of Gaussian errors, the results remain the same if the covariates are assumed to be random.



\subsection{Verification of (S3) and proof of Theorem \ref{theorem:theorem1} for double exponential errors}
\label{subsec:S3_de}
We now show that for all $\theta\in\Theta$, $\underset{n\rightarrow\infty}{\lim}\frac{1}{n}\log R_n(\theta)=-h(\theta)$, almost surely.
First note that 
\begin{align}
&\left|\frac{1}{n}R_n(\theta)+h(\theta)\right|\leq\left|\frac{1}{n}\sum_{i=1}^n\frac{|y_i-\eta_0(\bx_i)|}{\sigma_0}-1\right|\notag\\
&\quad+\left|\frac{1}{n}\sum_{i=1}^n\frac{|y_i-\eta(\bx_i)|}{\sigma}-\frac{1}{\sigma}E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|-
\frac{\sigma_0}{\sigma}E_{\bX}\left[\exp\left(-\frac{|\eta(\bX)-\eta_0(\bX)|}{\sigma_0}\right)\right]\right|.
\label{eq:h_de2}
\end{align}
Since $\frac{|y_i-\eta_0(\bx_i)|}{\sigma_0}$ has the exponential distribution with mean one, the term 
$\left|\frac{1}{n}\sum_{i=1}^n\frac{|y_i-\eta_0(\bx_i)|}{\sigma_0}-1\right|\rightarrow 0$ almost surely as $n\rightarrow\infty$ by the
strong law of large numbers.
That the term (\ref{eq:h_de2}) also tends to zero almost surely as $n\rightarrow\infty$ can be shown using the Borel-Cantelli lemma, using the inequality
(\ref{eq:bound3}), and replacing $\kappa_1$ in that inequality with any $\delta_1>0$.
In other words, it holds that for all $\theta\in\Theta$, $\underset{n\rightarrow\infty}{\lim}\frac{1}{n}\log R_n(\theta)=-h(\theta)$, almost surely.
Also, it follows from (\ref{eq:R_de}), (\ref{eq:lipcont_de}), (\ref{eq:h_de}), Lipschitz continuity of $x\mapsto\exp(-|x|)$, boundedness of the first derivative with respect to $\sigma$, 
that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is Lipschitz on $\theta\in\mathcal G_n\setminus I=\mathcal G_n$, which is compact. 
%Also, it is straightforward to directly verify, using the same techniques as (\ref{eq:lipcont_de}), that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is Lipschitz with respect to $\eta$.
%Since the function $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is also differentiable in $\sigma$, which is bounded in any $\mathcal G\in\left\{\mathcal G_1,\mathcal G_2,\ldots,\right\}$,
As a result, it follows that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is stochastically equicontinuous in $\mathcal G\in\left\{\mathcal G_1,\mathcal G_2,\ldots,\right\}$. Hence, the convergence  
$\underset{n\rightarrow\infty}{\lim}\frac{1}{n}\log R_n(\theta)=-h(\theta)$ occurs uniformly for $\theta\in\mathcal G$, almost surely.


\subsection{Verification of (S4)}
\label{subsec:S4_de}
Note that $h(\theta)\leq\log\left(\frac{\sigma}{\sigma_0}\right)-1+\frac{\|\eta-\eta_0\|+\sigma_0}{\sigma}$. Now $0<\|\eta-\eta_0\|<\infty$ and 
$0<\sigma<\infty$ with prior probability one. Consequently, it follows that
$h(\theta)<\infty$ with probability one, so that $I=\emptyset$ and hence, $\mathcal G_n\setminus I=\mathcal G_n$.

\subsection{Verification of (S5)}
\label{subsec:S5_de}

Verification of (S5) (1) and (S5) (2) remains the same as for Gaussian noise. (S5) (3) follows in the same way as for Gaussian noise is we can show that
$h(\theta)$ is continuous in $\theta$.
To see that $h(\theta)$ is continuous in $\theta$, again assume that $\eta_j\rightarrow\tilde\eta$ as $j\rightarrow\infty$ in the sense that $\|\eta_j-\tilde\eta\|\rightarrow 0$
as $j\rightarrow\infty$. Then $\left|E_{\bX}\left|\eta_j(\bX)-\eta_0(\bX)\right|-E_{\bX}\left|\tilde\eta(\bX)-\eta_0(\bX)\right|\right|\leq E_{\bX}\left|\eta_j(\bX)-\tilde\eta(\bX)\right|
\leq\|\eta_j-\tilde\eta\|\rightarrow 0$ as $j\rightarrow\infty$. Also, 
\begin{align}
&\left|E_{\bX}\left[\exp\left(-\frac{|\eta_j(\bX)-\eta_0(\bX)|}{\sigma_0}\right)\right]-E_{\bX}\left[\exp\left(-\frac{|\tilde\eta(\bX)-\eta_0(\bX)|}{\sigma_0}\right)\right]\right|\notag\\ 
&\leq E_{\bX}\left[\exp\left(-\left|\tilde\eta(\bX)-\eta_0(\bX)\right|\right)\times
\left|\exp\left(-\frac{\left(|\eta_j(\bX)-\eta_0(\bX)|-|\tilde\eta(\bX)-\eta_0(\bX)|\right)}{\sigma_0}\right)-1\right|\right]\notag\\
&\leq E_{\bX}\left[\exp\left(-\left|\tilde\eta(\bX)-\eta_0(\bX)\right|\right)\times
\left|\exp\left(\frac{|\eta_j(\bX)-\tilde\eta(\bX)|}{\sigma_0}\right)-1\right|\right]\notag\\
&\leq \left|\exp\left(\frac{\|\eta_j-\tilde\eta\|}{\sigma_0}\right)-1\right|\times E_{\bX}\left[\exp\left(-\left|\tilde\eta(\bX)-\eta_0(\bX)\right|\right)\right]\notag\\
&\rightarrow 0,~\mbox{as}~j\rightarrow\infty.\notag
\end{align}
Continuity of $h(\theta)$ hence follows easily.

\subsection{Verification of (S6) and proof of Theorem \ref{theorem:theorem3} for double exponential errors}
\label{subsec:S6_de}
It follows from (\ref{eq:h_de2}) that for all $\theta\in\Theta$, for $\kappa_1=\kappa-h(\Theta)$, we have
\begin{align}
&P\left(\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\kappa_1\right)
\leq P\left(\left|\frac{1}{\sigma_0}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta_0(\bx_i)\right|-1\right|>\frac{\kappa_1}{2}\right)\notag\\
&\qquad+P\left(\left|\frac{1}{\sigma}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|
-\frac{1}{\sigma}E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|\right.\right.\notag\\
&\qquad\qquad\qquad\left.\left.-\frac{\sigma_0}{\sigma}E_{\bX}\left(\exp\left\{-\frac{\left|\eta(\bX)-\eta_0(\bX)\right|}{\sigma_0}\right\}\right)\right|
>\frac{\kappa_1}{2}\right).
\label{eq:unif_de1}
\end{align}

%Now note that $Z_n=\frac{1}{\sigma_0}\sum_{i=1}^n\left|y_i-\eta_0(\bx_i)\right|\sim Gamma(n,1)$, where $Gamma(a,b)$ stands for the gamma distribution with mean $a/b$ and
%variance $a/b^2$. %Using the method of \ctn{Choi07} we obtain the following bound for the first term of the right hand side of (\ref{eq:unif_de1}):
Since $\frac{|y_i-\eta_0(\bx_i)|}{\sigma_0}$ are exponential random variables with expectation one, it follows that $\frac{|y_i-\eta_0(\bx_i)|}{\sigma_0}-1$ are zero-mean, 
independent sub-exponential random variables with some parameter $s>0$. Hence, by Bernstein's inequality (\ctn{Uspensky37}, \ctn{Bennett62}, \ctn{Massart03}),
\begin{align}
&P\left(\left|\frac{1}{\sigma_0}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta_0(\bx_i)\right|-1\right|>\frac{\kappa_1}{2}\right)
\leq 2\exp\left(-\frac{n}{2}\min\left\{\frac{\kappa^2_1}{4s^2},\frac{\kappa_1}{2s}\right\}\right).\notag
%=P\left(Z_n>n\left(1+\frac{\kappa_1}{2}\right)\right)+P\left(Z_n<n\left(1-\frac{\kappa_1}{2}\right)\right)\notag\\
%&\qquad\qquad\leq\exp\left\{-n\left(\frac{\kappa^2_1}{4}-\frac{\kappa^3_1}{6}\right)\right\}+\exp\left(-\frac{n\kappa^2_1}{4}\right).\notag
%\label{eq:gamma_de1}
\end{align}
Hence,
\begin{equation}
\int_{\mathcal S^c}P\left(\left|\frac{1}{\sigma_0}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta_0(\bx_i)\right|-1\right|>\frac{\kappa_1}{2}\right)
\leq 2\exp\left(-\frac{n}{2}\min\left\{\frac{\kappa^2_1}{4s^2},\frac{\kappa_1}{2s}\right\}\right).
\label{eq:summable1}
\end{equation}

%For the second term of the right hand side of (\ref{eq:unif_de1}), we make use of the following result presented in \ctn{Choi07}:
%\begin{lemma}[\ctn{Choi07}]
%\begin{itemize}
%\item[(a)]For every random variable $X$ with unimodal distribution symmetric around 0 and every $c\in\mathbb R$,
%\begin{equation}
%P\left((|X| \leq x\right) \geq P\left(|X + c| \leq x\right),~\forall x>0.
%\label{eq:choi1}
%\end{equation}
%\item[(b)]Let $X_1,\ldots,X_n$ and $Y_1,\ldots,Y_n$ be independent random variables. If
%$P\left(X_i \leq a\right) \leq P\left(Y_i\leq a\right)$,
%then, $\forall c \in\mathbb R$,
%\begin{equation}
%P\left(\sum_{i=1}^nX_i\leq c\right)\leq P\left(\sum_{i=1}^nX_i\leq c\right).
%\label{eq:choi2}
%\end{equation}
%\end{itemize}
%\end{lemma}
Let $\bar\varphi=E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|+\sigma_0E_{\bX}\left(\exp\left\{-\frac{\left|\eta(\bX)-\eta_0(\bX)\right|}{\sigma_0}\right\}\right)$. 
%Then using Jensen's inequality, 
%\begin{equation}
%\bar\varphi\geq \sigma_0\left[\frac{E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|}{\sigma_0}+\exp\left\{-\frac{E_{\bX}\left|\eta(\bX)-\eta_0(\bX)\right|}{\sigma_0}\right\}\right]\geq \sigma_0.
%\label{eq:jensen1}
%\end{equation}
Also, letting
$\varphi(\bx)=\left|\eta(\bx)-\eta_0(\bx)\right|+\sigma_0\left(\exp\left\{-\frac{\left|\eta(\bx)-\eta_0(\bx)\right|}{\sigma_0}\right\}\right)$, note that
\begin{equation}
\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)\rightarrow\bar\varphi,~\mbox{as}~n\rightarrow\infty.
\label{eq:varphi1}
\end{equation}
With this, the second term of (\ref{eq:unif_de1}) can be bounded as follows:
\begin{align}
&P\left(\left|\frac{1}{\sigma}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|-\frac{\bar\varphi}{\sigma}\right|>\frac{\kappa_1}{2}\right)\notag\\
%&\ \ \leq P\left(\left|\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|-\varphi\right|>\frac{\delta\xi}{2}\right)\notag\\
&\ \ = P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}+\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)-\bar\varphi\right|
>\frac{\kappa_1}{2}\right)\notag\\
&\ \ \leq P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}\right|>\frac{\kappa_1}{4}\right)
+P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)-\bar\varphi\right|>\frac{\kappa_1}{4}\right).
\label{eq:bound1}
\end{align}
%Now, due to (\ref{eq:varphi1}), there exists $n_0\geq 1$ such that for $n\geq n_0$, such that 
%\begin{equation}
%P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)-\bar\varphi\right|>\frac{\kappa_1}{4}\right)=0~\mbox{for}~n\geq n_0.
%\label{eq:bound2}
%\end{equation}
%In the case of random covariates $\bX$, it can be proved in the same way as (\ref{eq:bound_reference}), using the fact that 
%$\underset{\bx\in\mathcal X}{\sup}~\varphi(\bx) \leq \|\eta-\eta_0\|+\sigma_0$, that 
%$$P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)-\bar\varphi\right|>\frac{\delta}{4}\right)=O\left(n^{-3}\right).$$
%
In the case of random or non-random covariates $\bX$, again by Hoeffding's inequality,
\begin{equation}
P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)-\bar\varphi\right|>\frac{\kappa_1}{4}\right)
\leq \exp\left\{-\frac{n^2\kappa^2_1\sigma^2}{144nC^2}\right\}=\exp\left\{-\frac{n\kappa^2_1\sigma^2}{144C^2}\right\},
\label{eq:hoeff1}
\end{equation}
where $C>0$ is the upper bound of $|\varphi(\cdot)|$. Again, such an upper bound exists since $\mathcal X$ is compact and $\eta(\cdot)$ is continuous on $\mathcal X$.
%The same will be the bound for non-random covariates.
Application of the same method as proving (\ref{eq:term1_bound3_3}) yields
\begin{equation}
\int_{\mathcal S^c}P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\varphi(\bx_i)-\bar\varphi\right|>\frac{\kappa_1}{4}\right)\pi(\theta)d\theta
\leq c_3\exp\left[-\left(C_2\sqrt{\kappa_1n\psi_1}-3\sqrt{\beta n}-\tilde c_5n^q\right)\right],
\label{eq:summable2}
\end{equation}
where $\kappa_1$ is large enough to make the exponent of (\ref{eq:summable2}) negative.

For the first term of (\ref{eq:bound1}), let us first prove that $|y_i-\eta(\bx_i)|-\varphi(\bx_i)$ are sub-exponential random variables. Then we can apply Bernstein's
inequality to directly bound the term. %Indeed, straightforward calculation shows that for any $t>0$ such that $\sigma_0t<1$,
We need to show that $E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi(\bx_i)\right\}\right]\leq\exp\left(\frac{t^2s^2}{2}\right)$
for $|t|\leq s^{-1}$, for some $s>0$.

\subsection{Case 1: $t\geq 0$, $\eta(\bx_i)-\eta_0(\bx_i)>0$}
\label{subsec:case1}
Direct calculation shows that
\begin{align}
&E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi(\bx_i)\right\}\right]\notag\\
&=\exp\left(-t\varphi(\bx_i)\right)\times
\frac{\exp\left\{(\eta(\bx_i)-\eta_0(\bx_i))t\right\}-\exp\left(\frac{\eta_0(\bx_i)-\eta(\bx_i)}{\sigma_0}\right)}{1-\sigma^2_0t^2}\notag\\
&\leq\frac{\exp\left\{t\left(\varphi(\bx_i)+\eta(\bx_i)-\eta_0(\bx_i)\right)\right\}}{1-\sigma^2_0t^2}\notag\\
&\leq \frac{\exp\left\{t\left(2\|\eta-\eta_0\|+\sigma_0\right)\right\}}{1-\sigma^2_0t^2}.
\label{eq:subexp1}
\end{align}
To show that (\ref{eq:subexp1}) is bounded above by $\exp(t^2s^2/2)$, we need to show that 
\begin{equation}
f(t)=\frac{t^2s^2}{2}-2(\|\eta-\eta_0\|+\sigma_0)t+\log(1-\sigma^2_0t^2)\geq 0.
\label{eq:subexp2}
\end{equation}
For $t>0$, it is sufficient to show that 
\begin{equation}
\frac{ts^2}{2}\geq 2(\|\eta-\eta_0\|+\sigma_0)-\frac{\log(1-\sigma^2_0t^2)}{t}.
\label{eq:subexp3}
\end{equation}
Now, $-\frac{\log(1-\sigma^2_0t^2)}{t}\rightarrow 0$, as $t\rightarrow 0$. Hence, for any $\epsilon>0$, there exists $\delta(\epsilon)>0$ such that $t\leq\delta(\epsilon)$
implies $-\frac{\log(1-\sigma^2_0t^2)}{t}<\epsilon$. Let $s\geq\frac{C_1\|\eta-\eta_0\|+C_2}{\delta(\epsilon)}$, where $C_1>0$ and $C_2>0$ are sufficiently large quantities. 
Hence, if $\delta(\epsilon)^2\leq t\leq\delta(\epsilon)$, then (\ref{eq:subexp3}), and hence (\ref{eq:subexp2}), is satisfied. Now, $f(t)$ given by (\ref{eq:subexp2}) is continuous in $t$
and $f(0)=0$. Hence, (\ref{eq:subexp2}) holds even for $0\leq t\leq\delta(\epsilon)^2$. In other words,
\begin{equation}
E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi\right\}\right]\leq\exp\left(\frac{t^2s^2}{2}\right),~\mbox{for}~0\leq t\leq s^{-1}
\leq\frac{\delta(\epsilon)}{C_1\|\eta-\eta_0\|+C_2}\leq\delta(\epsilon).
\label{eq:subexp4}
\end{equation}


\subsection{Case 2: $t\geq 0$, $\eta(\bx_i)-\eta_0(\bx_i)<0$}
\label{subsec:case2}
In this case,
\begin{align}
&E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi(\bx_i)\right\}\right]\notag\\
&=\exp\left(-t\varphi(\bx_i)\right)\times
\frac{\exp\left\{(\eta_0(\bx_i)-\eta(\bx_i))t\right\}+\sigma_0t\exp\left(\frac{\eta(\bx_i)-\eta_0(\bx_i)}{\sigma_0}\right)}{1-\sigma^2_0t^2}\notag\\
&\leq \exp\left(t\varphi(\bx_i)\right)\times
\frac{2\exp\left\{(\eta_0(\bx_i)-\eta(\bx_i))t\right\}}{1-\sigma^2_0t^2}\notag\\
&\leq\frac{\exp\left\{t\left(\varphi(\bx_i)+(\eta_0(\bx_i)-\eta(\bx_i))\right)\right\}}{\frac{1-\sigma^2_0t^2}{2}}\notag\\
&\leq \frac{\exp\left\{t\left(2\|\eta-\eta_0\|+\sigma_0\right)\right\}}{\frac{1-\sigma^2_0t^2}{2}}.\notag
%\label{eq:subexp5}
\end{align}
As in Section \ref{subsec:case1} it can be seen that (\ref{eq:subexp4}) holds.

\subsection{Case 3: $t\leq 0$, $\eta(\bx_i)-\eta_0(\bx_i)>0$}
\label{subsec:case3}
Here
\begin{align}
&E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi(\bx_i)\right\}\right]\notag\\
&=\exp\left(-t\varphi(\bx_i)\right)\times
\frac{\exp\left\{(\eta(\bx_i)-\eta_0(\bx_i))t\right\}-\sigma_0|t|\exp\left(\frac{\eta_0(\bx_i)-\eta(\bx_i)}{\sigma_0}\right)}{1-\sigma^2_0t^2}\notag\\
&\leq \exp\left(-t\varphi(\bx_i)\right)\times
\frac{1}{1-\sigma^2_0t^2}\notag\\
&\leq \frac{\exp\left\{-t\left(\|\eta-\eta_0\|+\sigma_0\right)\right\}}{1-\sigma^2_0t^2}.\notag
%\label{eq:subexp6}
\end{align}
Here we need to have
$|t|\left[\frac{|t|s^2}{2}-\left(\|\eta-\eta_0\|+\sigma_0\right)+\frac{\log(1-\sigma^2_0t^2)}{|t|}\right]>0$. In the same way as before it follows that
\begin{equation}
E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi\right\}\right]\leq\exp\left(\frac{t^2s^2}{2}\right),~\mbox{for}~0\leq |t|\leq s^{-1}
\leq\frac{\delta(\epsilon)}{C_1\|\eta-\eta_0\|+C_2}\leq\delta(\epsilon).\notag
\label{eq:subexp7}
\end{equation}


\subsection{Case 4: $t\leq 0$, $\eta(\bx_i)-\eta_0(\bx_i)<0$}
\label{subsec:case4}
In this case,
\begin{align}
&E_{\theta_0}\left[\exp\left\{t\left(|y_i-\eta(\bx_i)|\right)-\varphi(\bx_i)\right\}\right]\notag\\
&=\exp\left(-t\varphi(\bx_i)\right)\times
\frac{\exp\left\{(\eta_0(\bx_i)-\eta(\bx_i))t\right\}-\sigma_0|t|\exp\left(\frac{\eta(\bx_i)-\eta_0(\bx_i)}{\sigma_0}\right)}{1-\sigma^2_0t^2}\notag\\
&\leq \exp\left(-t\varphi(\bx_i)\right)\times
\frac{1}{1-\sigma^2_0t^2}\notag\\
&\leq \frac{\exp\left\{-t\left(\|\eta-\eta_0\|+\sigma_0\right)\right\}}{1-\sigma^2_0t^2}.\notag
%\label{eq:subexp8}
\end{align}
Hence, (\ref{eq:subexp7}) holds.


Hence, for $i=1,\ldots,n$, $|y_i-\eta(\bx_i)|-E\left(|y_i-\eta(\bx_i)|\right)$ are 
zero-mean, independent sub-exponential random variables with parameter $s$. In particular, we can set $s=\frac{C_1\|\eta-\eta_0\|+C_2}{\delta(\epsilon)}$. Hence, by Bernstein's inequality,
\begin{align}
&P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}\right|>\frac{\kappa_1}{4}\right)\notag\\
&\leq 2\max\left\{P\left(\frac{\sigma^{-1}}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}>\frac{\kappa_1}{4}\right),
P\left(\frac{\sigma^{-1}}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}< -\frac{\kappa_1}{4}\right)\right\}\notag\\
&\leq 2\exp\left(-\frac{n}{2}\min\left\{\frac{\kappa^2_1\sigma^2}{16s^2},\frac{\kappa_1\sigma}{4s}\right\}\right)\notag\\
&=2\exp\left(-\frac{n}{2}\min\left\{\frac{\kappa^2_1\delta(\epsilon)^2\sigma^2}{16(C_1\|\eta-\eta_0\|+C_2)^2},\frac{\kappa_1\delta(\epsilon)\sigma}{4(C_1\|\eta-\eta_0\|+C_2)}\right\}\right).
\label{eq:bound3}
\end{align}
Applying the same techniques of proving (\ref{eq:zero_prob4}) and (\ref{eq:zero_prob5}) to (\ref{eq:bound3}), it is easy to see that
\begin{align}
&P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}\right|>\frac{\kappa_1}{4}\right)\notag\\
&\leq\tilde C_1\exp\left\{-\left(\kappa_1\tilde C_2\sqrt{n\psi_1}-\tilde C_3\sqrt{\beta n}-\tilde C_4 n^q\right)\right\}\notag\\
&\qquad+\tilde C_5\exp\left\{-\left(\tilde C_6\sqrt{\kappa_1n\psi_2}-\tilde C_7\sqrt{\beta n}-\tilde C_8 n^q\right)\right\}+2\pi\left(\mathcal G^c_n\right).
\label{eq:summable3}
\end{align}

\begin{comment}
note that by Markov's inequality,
\begin{align}
&P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}\right|>\frac{\delta}{4}\right)\notag\\
&\ \ \leq n^{-6}\left(\frac{\delta}{4}\right)^{-6}E_{\theta_0}\left(\sum_{i=1}^n\sigma^{-1}\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}\right)^6
= n^{-6}\left(\frac{\delta\xi}{4}\right)^{-6}E_{\theta_0}\left(\sum_{i=1}^n\tilde y_i\right)^6,
\label{eq:bound3}
\end{align}
where $\tilde y_i=\frac{\left|y_i-\eta(\bx_i)\right|}{\sigma}-\frac{\varphi(\bx_i)}{\sigma}$. Note that $E_{\theta_0}(\tilde y_i)=0$, for $i=1,\ldots,n$.
Now, by independence among $\left\{\tilde y_i:i=1,\ldots,n\right\}$, 
$E_{\theta_0}\left(\sum_{i=1}^n\tilde y_i\right)^6=\sum_{b_1+\cdots+b_n=6}\prod_{i=1}^nE_{\theta_0}\left(\tilde y_i\right)^{b_i}$, for non-negative integers $b_1,\ldots,b_n$.
Now $\prod_{i=1}^nE_{\theta_0}\left(\tilde y_i\right)^{b_i}\neq 0$ in four cases. These are (i) one of the $b_i=6$ and $b_j=0$ for $j\neq i$; (ii) one of the $b_i=4$, another
$b_j=2$, for $j\neq i$, and $b_k=0$, for $k\neq j\neq i$; (iii) $b_i=b_j=3$, for some $i\neq j$, and $b_k=0$, for $k\neq j\neq i$; 
(iv) $b_i=b_j=b_k=2$, for some $i\neq j\neq k$, and $b_l=0$, for $l\neq k\neq j\neq i$. The number of possible situations favourable to the four cases are $n$, $n(n-1)$, $\frac{n(n-1)}{2}$
and $\frac{n(n-1)(n-2)}{6}$, respectively. Now note that for $b\geq 2$, and for any $\bx\in\mathcal X$,
\begin{align}
&E_{\theta_0}\left|\frac{y-\eta(\bx)}{\sigma}\right|^b\notag\\
&=\frac{1}{2\sigma_0}\int\left|\frac{y-\eta(\bx)}{\sigma}\right|^b\exp\left(-\frac{|y-\eta_0(\bx)|}{\sigma_0}\right)dy\notag\\
&=\frac{1}{2\sigma_0}\int\left|\frac{z+\eta_0(\bx)-\eta(\bx)}{\sigma}\right|^b\exp\left(-\frac{|z|}{\sigma_0}\right)dz\notag\\
&\leq\frac{1}{2\sigma_0}\int\left(\frac{|z|+|\eta_0(\bx)-\eta(\bx)|}{\sigma}\right)^b\exp\left(-\frac{|z|}{\sigma_0}\right)dz\notag\\
&\leq\frac{1}{2\sigma_0}\int\left(\frac{|z|+\|\eta-\eta_0\|}{\sigma}\right)^b\exp\left(-\frac{|z|}{\sigma_0}\right)dz.
%&\leq\frac{1}{2\sigma_0}\int\left(\frac{|z|+\kappa_0}{\xi}+\frac{1}{\kappa_1}\right)^b\exp\left(-\frac{|z|}{\sigma_0}\right)dz
%~\left(\mbox{since}~\sigma>\xi~\mbox{and}~\frac{\|\eta-\eta_0\|}{\sigma}%\leq \frac{\|\eta\|}{\sigma}+\frac{\|\eta_0\|}{\sigma}
%\leq\frac{1}{\kappa_1}+\frac{\kappa_0}{\xi}\right).
\label{eq:uniform_bound}
\end{align}

Since the relevant values of $b_i$ are less than or equal to 6, 
it follows from (\ref{eq:uniform_bound}) that 
$E_{\theta_0}\left(\tilde y_i\right)^{b_i}$ is uniformly bounded with respect to $i$.
%thanks to finiteness of the norms of $\eta$ and $\eta_0$ and since
%$\exp\left(-\frac{\left|\eta(\bx)-\eta_0(\bx)\right|}{\sigma_0}\right)\leq 1$ for all $\bx$. 
Consequently we deduce that (\ref{eq:bound3}) is given by: %$O\left(\frac{n+2n(n-1)+n(n-1)(n-2)}{n^6}\right)=O\left(n^{-3}\right)$.
\begin{equation}
P\left(\sigma^{-1}\left|\frac{1}{n}\sum_{i=1}^n\left\{\left|y_i-\eta(\bx_i)\right|-\varphi(\bx_i)\right\}\right|>\frac{\delta}{4}\right)=O\left(n^{-3}\right).
\label{eq:bound_reference}
\end{equation}
Hence, the second term of (\ref{eq:unif_de1}) is given by:
\begin{equation}
P\left(\left|\frac{1}{\sigma}\times\frac{1}{n}\sum_{i=1}^n\left|y_i-\eta(\bx_i)\right|-\frac{\bar\varphi}{\sigma}\right|>\frac{\delta}{2}\right)=O\left(n^{-3}\right).
\label{eq:bound4}
\end{equation}

\end{comment}



Gathering (\ref{eq:summable1}), (\ref{eq:summable2}) and (\ref{eq:summable3}) we see that
for all $\theta\in\Theta$, for any $\delta>0$, and for some $a>0$,
\begin{equation}
\sum_{n=1}^{\infty}\int_{\mathcal S^c}P\left(\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|>\delta\right)\pi(\theta)d\theta<\infty.
\label{eq:unif_de2}
\end{equation}
%The proof of uniform convergence of (\ref{eq:uniform_conv_de}) over $\mathcal G_n\setminus I$ as required by (S5) (2) follows from the proof of (\ref{eq:uniform_conv_de}). 
%Indeed, it follows from (\ref{eq:R_de}), (\ref{eq:lipcont_de}), (\ref{eq:h_de}), Lipschitz continuity of $x\mapsto\exp(-|x|)$, boundedness of the first derivative with respect to $\sigma$, 
%that $\frac{1}{n}\log R_n(\theta)+h(\theta)$ is Lipschitz on $\theta\in\mathcal G_n\setminus I=\mathcal G_n$, which is compact. 
%Hence, combined with the proof of (\ref{eq:uniform_conv_de}), these guarantee (S5) (2).
%so that 
%$\underset{\theta\in\mathcal G_n}{\sup}~\left|\frac{1}{n}\log R_n(\theta)+h(\theta)\right|
%=\left|\frac{1}{n}\log R_n(\hat\theta)+h(\hat\theta)\right|$, for some $\hat\theta\in\mathcal G_n$, perhaps depending on the data. Since (\ref{eq:unif_de2}) holds for all $\theta\in\Theta$
%and that the upper bound is independent of $\theta$,
%the same must hold for $\theta=\hat\theta$.

\subsection{Verification of (S7)}
\label{subsec:S7_de}
Verification of (S7) is exactly the same as for Gaussian errors.


